Automatic Specialization of Third-Party Java Dependencies

Large-scale code reuse significantly reduces both development costs and time. However, the massive share of third-party code in software projects poses new challenges, especially in terms of maintenance and security. In this paper, we propose a novel technique to specialize dependencies of Java projects, based on their actual usage. Given a project and its dependencies, we systematically identify the subset of each dependency that is necessary to build the project, and we remove the rest. As a result of this process, we package each specialized dependency in a JAR file. Then, we generate specialized dependency trees where the original dependencies are replaced by the specialized versions. This allows building the project with significantly less third-party code than the original. As a result, the specialized dependencies become a first-class concept in the software supply chain, rather than a transient artifact in an optimizing compiler toolchain. We implement our technique in a tool called DepTrim, which we evaluate with 30 notable open-source Java projects. DepTrim specializes a total of 343 (86.6%) dependencies across these projects, and successfully rebuilds each project with a specialized dependency tree. Moreover, through this specialization, DepTrim removes a total of 57,444 (42.2%) classes from the dependencies, reducing the ratio of dependency classes to project classes from 8.7x in the original projects to 5.0x after specialization. These novel results indicate that dependency specialization significantly reduces the share of third-party code in Java projects.

==> compilation_errors_logs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%
% checkstyle
%%%%%%%%%%%%%%%%%%%%%%%%%
commons-beanutils

[INFO] -------------------------------------------------------------
[ERROR] COMPILATION ERROR : 
[INFO] -------------------------------------------------------------
[ERROR] /Users/cesarsv/IdeaProjects/deptrim-experiments/pipeline/projects/checkstyle/src/test/resources/com/puppycrawl/tools/checkstyle/checks/whitespace/emptylineseparator/InputEmptyLineSeparator2.java:[29,54] package org.apache.commons.beanutils.locale.converters does not exist
[ERROR] /Users/cesarsv/IdeaProjects/deptrim-experiments/pipeline/projects/checkstyle/src/test/resources/com/puppycrawl/tools/checkstyle/checks/whitespace/emptylineseparator/InputEmptyLineSeparator2.java:[30,36] cannot find symbol
  symbol:   class BasicDynaBean
  location: package org.apache.commons.beanutils

guava

[ERROR] COMPILATION ERROR : 
[INFO] -------------------------------------------------------------
[ERROR] /Users/cesarsv/IdeaProjects/deptrim-experiments/pipeline/projects/checkstyle/src/main/java/com/puppycrawl/tools/checkstyle/utils/ModuleReflectionUtil.java:[29,33] package com.google.common.reflect does not exist
[ERROR] /Users/cesarsv/IdeaProjects/deptrim-experiments/pipeline/projects/checkstyle/src/main/java/com/puppycrawl/tools/checkstyle/utils/ModuleReflectionUtil.java:[59,15] cannot find symbol
  symbol:   class ClassPath
  location: class com.puppycrawl.tools.checkstyle.utils.ModuleReflectionUtil
[ERROR] /Users/cesarsv/IdeaProjects/deptrim-experiments/pipeline/projects/checkstyle/src/main/java/com/puppycrawl/tools/checkstyle/utils/ModuleReflectionUtil.java:[59,37] cannot find symbol
  symbol:   variable ClassPath
  location: class com.puppycrawl.tools.checkstyle.utils.ModuleReflectionUtil
  
%%%%%%%%%%%%%%%%%%%%%%
% Chronicle-map
%%%%%%%%%%%%%%%%%%%%%%
pax-url-aether

[ERROR] COMPILATION ERROR : 
[INFO] -------------------------------------------------------------
[ERROR] /home/ubuntu/cesarsv/pipeline/projects/Chronicle-Map/src/test/java/net/openhft/chronicle/map/LostKeyTest.java:[36,31] cannot access shaded.org.apache.commons.codec.BinaryEncoder
  class file for shaded.org.apache.commons.codec.BinaryEncoder not found


%%%%%%%%%%%%%%%%%%%%%%
% flink
%%%%%%%%%%%%%%%%%%%%%%
flink-core

[ERROR] COMPILATION ERROR : 
[INFO] -------------------------------------------------------------
[ERROR] /home/ubuntu/cesarsv/pipeline/projects/flink/flink-java/src/test/java/org/apache/flink/api/common/io/SerializedFormatTest.java:[55,15] cannot find symbol
  symbol:   class SerializedInputFormat
  location: class org.apache.flink.api.common.io.SerializedFormatTest

%%%%%%%%%%%%%%%%%%%%%%
% graphhopper
%%%%%%%%%%%%%%%%%%%%%%
<dependency>
      <groupId>se.kth.castor.deptrim.spl</groupId>
      <artifactId>graphhopper-web-api</artifactId>
      <version>6.0-SNAPSHOT</version>
      <scope>compile</scope>
      <optional>false</optional>
</dependency>

[WARNING] The POM for se.kth.castor.deptrim.spl:graphhopper-web-api:jar:6.0-SNAPSHOT is missing, no dependency information available
[INFO] ------------------------------------------------------------------------
[INFO] BUILD FAILURE
[INFO] ------------------------------------------------------------------------
[INFO] Total time:  0.398 s
[INFO] Finished at: 2023-01-21T19:33:36+01:00
[INFO] ------------------------------------------------------------------------
[ERROR] Failed to execute goal on project graphhopper-core: Could not resolve dependencies for project com.graphhopper:graphhopper-core:jar:6.0-SNAPSHOT: Could not find artifact se.kth.castor.deptrim.spl:graphhopper-web-api:jar:6.0-SNAPSHOT -> [Help 1]
[ERROR] 


%%%%%%%%%%%%%%%%%%%%%%
% helidon
%%%%%%%%%%%%%%%%%%%%%%
<dependency>
    <groupId>se.kth.castor.deptrim.spl</groupId>
    <artifactId>smallrye-open-api-core</artifactId>
    <version>2.0.26</version>
    <scope>compile</scope>
    <optional>false</optional>
</dependency>

[INFO] BUILD FAILURE
[INFO] ------------------------------------------------------------------------
[INFO] Total time:  3.548 s
[INFO] Finished at: 2023-01-25T11:32:14Z
[INFO] ------------------------------------------------------------------------
[ERROR] Failed to execute goal io.helidon.build-tools:snakeyaml-codegen-maven-plugin:2.3.7:generate (generate-snakeyaml-parsing-helper) on project helidon-openapi: Cannot find specified inputDirectory /home/ubuntu/cesarsv/pipeline/projects/helidon/openapi/target/extracted-sources/openapi-impls -> [Help 1]
[ERROR] 


%%%%%%%%%%%%%%%%%%%%%%
% jacop
%%%%%%%%%%%%%%%%%%%%%%
<dependency>
  <groupId>se.kth.castor.deptrim.spl</groupId>
  <artifactId>mockito-all</artifactId>
  <version>1.10.19</version>
  <scope>compile</scope>
  <optional>false</optional>
</dependency>

[INFO] ------------------------------------------------------------------------
[INFO] BUILD FAILURE
[INFO] ------------------------------------------------------------------------
[INFO] Total time:  56.908 s
[INFO] Finished at: 2023-01-06T12:43:32+01:00
[INFO] ------------------------------------------------------------------------
[ERROR] Failed to execute goal org.apache.maven.plugins:maven-compiler-plugin:3.8.1:testCompile (default-testCompile) on project jacop: Compilation failure: Compilation failure: 
[ERROR] /Users/cesarsv/IdeaProjects/deptrim-experiments/pipeline/projects/jacop/src/test/java/org/jacop/IntDomainTest.java:[48,26] cannot find symbol
[ERROR]   symbol:   class MockitoAnnotations
[ERROR]   location: package org.mockito


%%%%%%%%%%%%%%%%%%%%%%
% javafaker
%%%%%%%%%%%%%%%%%%%%%%
<dependency>
  <groupId>se.kth.castor.deptrim.spl</groupId>
  <artifactId>snakeyaml</artifactId>
  <version>1.26</version>
  <classifier>android</classifier>
  <scope>compile</scope>
  <optional>false</optional>
</dependency>

Downloading from central: https://repo.maven.apache.org/maven2/se/kth/castor/deptrim/spl/snakeyaml/1.26/snakeyaml-1.26-android.jar
[INFO] ------------------------------------------------------------------------
[INFO] BUILD FAILURE
[INFO] ------------------------------------------------------------------------
[INFO] Total time:  1.801 s
[INFO] Finished at: 2023-01-06T13:09:31+01:00
[INFO] ------------------------------------------------------------------------
[ERROR] Failed to execute goal on project javafaker: Could not resolve dependencies for project com.github.javafaker:javafaker:jar:1.0.3-SNAPSHOT: Could not find artifact se.kth.castor.deptrim.spl:snakeyaml:jar:android:1.26 in central (https://repo.maven.apache.org/maven2) -> [Help 1]
[ERROR] 

%%%%%%%%%%%%%%%%%%%%%%
% jcabi-github
%%%%%%%%%%%%%%%%%%%%%%
<dependency>
      <groupId>se.kth.castor.deptrim.spl</groupId>
      <artifactId>jcabi-http</artifactId>
      <version>1.20.1</version>
      <scope>compile</scope>
      <exclusions>
        <exclusion>
          <groupId>com.jcabi</groupId>
          <artifactId>jcabi-manifests</artifactId>
        </exclusion>
      </exclusions>
      <optional>false</optional>
 </dependency>
 
[INFO] ------------------------------------------------------------------------
[INFO] BUILD FAILURE
[INFO] ------------------------------------------------------------------------
[INFO] Total time:  8.310 s
[INFO] Finished at: 2023-01-07T11:08:23+01:00
[INFO] ------------------------------------------------------------------------
[ERROR] Failed to execute goal org.apache.maven.plugins:maven-compiler-plugin:3.10.1:testCompile (default-testCompile) on project jcabi-github: Compilation failure: Compilation failure: 
[ERROR] /Users/cesarsv/IdeaProjects/deptrim-experiments/pipeline/projects/jcabi-github/src/test/java/com/jcabi/github/RtPaginationTest.java:[127,29] cannot access com.jcabi.http.mock.MkAnswer.Simple
[ERROR]   class file for com.jcabi.http.mock.MkAnswer$Simple not found

%%%%%%%%%%%%%%%%%%%%%%
% jooby
%%%%%%%%%%%%%%%%%%%%%%
<dependency>
    <groupId>se.kth.castor.deptrim.spl</groupId>
    <artifactId>kotlinx-coroutines-core-jvm</artifactId>
    <version>1.6.2</version>
    <scope>compile</scope>
    <optional>true</optional>
</dependency>

[INFO] ------------------------------------------------------------------------
[INFO] BUILD FAILURE
[INFO] ------------------------------------------------------------------------
[INFO] Total time:  02:06 min
[INFO] Finished at: 2023-01-17T21:42:01+01:00
[INFO] ------------------------------------------------------------------------
[ERROR] Failed to execute goal org.jetbrains.kotlin:kotlin-maven-plugin:1.6.21:test-compile (test-compile) on project jooby: Compilation failure: Compilation failure: 
[ERROR] /Users/cesarsv/IdeaProjects/deptrim-experiments/pipeline/projects/jooby/jooby/src/test/kotlin/apps/Apps.kt:[6,27] Unresolved reference: delay
[ERROR] /Users/cesarsv/IdeaProjects/deptrim-experiments/pipeline/projects/jooby/jooby/src/test/kotlin/apps/Apps.kt:[15,7] Unresolved reference: delay
[ERROR] /Users/cesarsv/IdeaProjects/deptrim-experiments/pipeline/projects/jooby/jooby/src/test/kotlin/apps/Apps.kt:[46,9] Unresolved reference: delay
[ERROR] /Users/cesarsv/IdeaProjects/deptrim-experiments/pipeline/projects/jooby/jooby/src/test/kotlin/io/jooby/CoroutineRouterTest.kt:[5,27] Unresolved reference: coroutineScope
[ERROR] /Users/cesarsv/IdeaProjects/deptrim-experiments/pipeline/projects/jooby/jooby/src/test/kotlin/io/jooby/CoroutineRouterTest.kt:[40,9] Unresolved reference. None of the following candidates is applicable because of receiver type mismatch: 
[ERROR] public operator fun <T, R> DeepRecursiveFunction<TypeVariable(T), TypeVariable(R)>.invoke(value: TypeVariable(T)): TypeVariable(R) defined in kotlin
[ERROR] /Users/cesarsv/IdeaProjects/deptrim-experiments/pipeline/projects/jooby/jooby/src/test/kotlin/io/jooby/CoroutineRouterTest.kt:[41,27] Unresolved reference: coroutineContext
[ERROR] /Users/cesarsv/IdeaProjects/deptrim-experiments/pipeline/projects/jooby/jooby/src/test/kotlin/io/jooby/Idioms.kt:[5,27] Unresolved reference: delay
[ERROR] /Users/cesarsv/IdeaProjects/deptrim-experiments/pipeline/projects/jooby/jooby/src/test/kotlin/io/jooby/Idioms.kt:[130,7] Unresolved reference: delay


%%%%%%%%%%%%%%%%%%%%%%
% OpenPDF
%%%%%%%%%%%%%%%%%%%%%%
<dependency>
      <groupId>se.kth.castor.deptrim.spl</groupId>
      <artifactId>fop</artifactId>
      <version>2.7</version>
      <scope>compile</scope>
      <exclusions>
        <exclusion>
          <groupId>org.apache.xmlgraphics</groupId>
          <artifactId>fop-util</artifactId>
        </exclusion>
        <exclusion>
          <groupId>org.apache.xmlgraphics</groupId>
          <artifactId>fop-events</artifactId>
        </exclusion>
      </exclusions>
      <optional>true</optional>
</dependency>

[ERROR] COMPILATION ERROR : 
[INFO] -------------------------------------------------------------
[ERROR] /home/dee/dev/deptrim-experiments/pipeline/projects/OpenPDF/openpdf/src/main/java9/module-info.java:[4,21] module not found: fop
[INFO] 1 error
[INFO] -------------------------------------------------------------
[INFO] ------------------------------------------------------------------------
[INFO] BUILD FAILURE
[INFO] ------------------------------------------------------------------------
[INFO] Total time:  9.013 s
[INFO] Finished at: 2023-01-22T14:49:53+01:00
[INFO] ------------------------------------------------------------------------
[ERROR] Failed to execute goal org.apache.maven.plugins:maven-compiler-plugin:3.10.1:compile (compile-java-9) on project openpdf: Compilation failure
[ERROR] /home/dee/dev/deptrim-experiments/pipeline/projects/OpenPDF/openpdf/src/main/java9/module-info.java:[4,21] module not found: fop



%%%%%%%%%%%%%%%%%%%%%%
% woodstox
%%%%%%%%%%%%%%%%%%%%%%
<dependency>
      <groupId>se.kth.castor.deptrim.spl</groupId>
      <artifactId>stax2-api</artifactId>
      <version>4.2.1</version>
      <scope>compile</scope>
      <optional>false</optional>
</dependency>
    
[INFO] ------------------------------------------------------------------------
[INFO] BUILD FAILURE
[INFO] ------------------------------------------------------------------------
[INFO] Total time:  16.628 s
[INFO] Finished at: 2023-01-06T13:45:29+01:00
[INFO] ------------------------------------------------------------------------
[ERROR] Failed to execute goal org.apache.maven.plugins:maven-compiler-plugin:3.10.1:testCompile (default-testCompile) on project woodstox-core: Compilation failure: Compilation failure: 
[ERROR] /Users/cesarsv/IdeaProjects/deptrim-experiments/pipeline/projects/woodstox/src/test/java/stax2/wstream/TestWriterConstruction.java:[22,61] cannot find symbol
[ERROR]   symbol:   class Stax2FileResult
[ERROR]   location: class stax2.wstream.TestWriterConstruction


==> csv-notes.tex <==
\subsection{Specialization in the Modern Java Ecosystem}\label{sec:spec}

%  A paragraph explaining that most of the code is actually in the dependencies.
Modern software development relies heavily on the reuse of third-party dependencies. 
As of January 2023~\cite{MavenRepository2023}, the Maven Central Repository has more than \np[M]{10} indexed artifacts.
Each artifact provides pre-built functionalities that can be easily integrated into a project, reducing developer effort.
% the amount of code that needs to be written and maintained by developers. 
The use of dependencies allows developers to take advantage of existing solutions to common problems, which can save time, resources, and increase the reliability of their codebase.
% Many libraries and frameworks are open-source and are actively managed by a community of developers.
In fact, most of the code that is packaged in a typical Java application is not developed directly by the authors of the application, but added via third-party dependencies.
Despite the benefits of using dependencies, this situation needlessly increases the size of the packaged project and its attack surface, degrades build performance, and affects maintainability.

% A paragraph introducing GraalVM as the avant grade solution to the previous situation.
The Java community is currently taking action to mitigate the adverse effects of dependency usage.
The GraalVM native image compiler~\cite{ProjectLeyden2022} embraces Ahead of Time Compilation (AOT) to statically transform bytecode directly into machine code at build time (\ie, before execution)~\cite{GraalVMNativeImage2023}.
To do so, the GraalVM performs aggressive optimizations such as the elimination of unused code from the bytecode of Java projects, their dependencies, as well as the JDK. 
This produces a self-contained native executable that only includes code that is actually necessary to build and execute a project. 
The result is a native image executable with high performance and less memory overhead, leading to smaller container images. 
This optimal resource consumption with less CPU and memory is ideal for the cloud, making Java applications easy to ship and deploy directly (\eg, as in a microservices-based architecture).

% A paragraph describing the current limitations of GraalVM
The GraalVM native image technology relies on static analysis to build a native executable that only includes the elements reachable from an application entry point, its dependencies, and the JDK classes discovered.
To do so, the points-to analysis of the AOT compilation needs to “reach” all the bytecode to work correctly~\cite{wimmer2021graalvm}. 
This means that all the bytecode in the application and their dependencies that can be called at runtime must be known at build time (observed and analyzed), \ie, when the native-image tool in GraalVM is building the standalone executable.
This limitation is known as the \emph{closed-world assumption}~\cite{Wimmer2019}. 
The reachability of some elements (such as classes, methods, or fields) may not be discoverable due to the Java dynamic features, \eg, reflection, resource access, dynamic proxies, and serialization~\cite{sui2018soundness, landman2017challenges,li2019understanding, reif2019judge}.
Consequently, dynamic language capabilities such as Java Native Interface (JNI), Java Reflection, Dynamic Proxy objects (\texttt{java.lang.reflect.Proxy}), or classpath resources (\texttt{Class.getResource}) are not supported.
The closed-world constraint imposes strict limits on Java’s natural dynamism, particularly on the run-time reflection and class-loading features upon which so many existing Java libraries and frameworks depend. 
For the time being, not all applications are well suited to this constraint, and not all developers are willing to live with it.

% A paragraph about the need to use a gradual incremental approach to port the dependencies that are affected by the limitations
If an element is not reachable, it is not included in the generated executable and this can lead to runtime failures. 
To include elements whose reachability is undiscoverable, the native image builder requires externally provided reachability metadata.
To mitigate this limitation, GraalVM provides a tracing Java agent that tracks all usages of dynamic features utilized by a running JVM.
This agent interfaces with the JVM at runtime and intercepts all calls that look up classes, methods, fields, resources, or request proxy accesses. 
The agent then writes a report with all the intercepted dynamic accesses. 
This report can be passed to the native-image tool so that the used classes will not be removed during the image build process.


Therefore, rather than adopt the closed-world constraint at the start, the Java community instead pursues a gradual, incremental approach.
Today the community works incrementally along this spectrum of constraints, starting small and simple in order to develop a firm understanding of the changes required to the Java Platform Specification. while preserving Java’s core values of readability, compatibility, and generality. 
In the long run, Java will likely embrace the full closed-world constraint in order to produce fully-static images. 
Between now and then, however, the community works on developing and delivering incremental improvements which developers can use sooner rather than later.
A notable effort is the GraalVM Reachability Metadata Repository~\cite{GraalVMReachabilityMetadata2023}, which enables native image users to share and reuse metadata for libraries and frameworks in the Java ecosystem, and thus simplify maintaining third-party dependencies. 
The repository is integrated with GraalVM Native Build Tools beginning with version \texttt{0.9.13}, and integrates with notable Java web frameworks such as Spring Boot 3.0, Quarkus, and Micronaut~\cite{vsipek2020enhancing}.

% The future is with GraalVM, but meanwhile, we need DepTrim
GraalVM and native image compilation is perceived by many as the future of JVM-based languages.
However, since the native image creation process analyzes the bytecode in the application and all its dependencies, there is a risk of violating the close world if at least one of the dependencies relies on some dynamic Java feature. 
The community is creating new versions of libraries that respect this assumption. 
However, there is still insufficient support for the most popular Java libraries. 
This technology still needs some time to mature before its massive adoption.
In this paper, we introduce a novel technique to specialize the third-party dependencies of Java applications by removing unnecessary classes. 
Our approach is unique in the sense that it takes into account the fact that many dependencies may violate the close world assumption.

==> graalvm-text.tex <==
\subsection{Specialization in the Modern Java Ecosystem}\label{sec:spec}

% A paragraph introducing GraalVM as the avant grade solution to the previous situation.
The Java community is currently making efforts to mitigate the adverse impacts of dependency usage.
The existing \texttt{maven-shade-plugin} produces a fat \jar by extracting the content of the dependencies and adding them along the packaged classes and resources of the project itself, resulting in a big \jar.
This way, having a single \jar facilitates deployment, execution, and distribution in some cases.
However, a fat \jar is not appropriate for reuse as it cancels the purpose of the dependency resolution mechanism of \maven.
Therefore, the \texttt{maven-shade-plugin} is typically used for final deployment.
% In contrast, \deptrim modifies the content of each dependency separately and deploys them in the local repository.
% Furthermore, \deptrim produces a modified version of the \pom file that reuses the dependencies without altering the packaged \jar of the project.
% This procedure facilitates reuse and keeps the dependency resolution mechanism. 

The GraalVM native image compiler~\cite{ProjectLeyden2022} embraces Ahead of Time Compilation (AOT) to statically transform bytecode directly into machine code at build time (\ie, before execution)~\cite{GraalVMNativeImage2023}.
To do so, the GraalVM performs aggressive optimizations such as the elimination of unused code from the bytecode of Java projects, their dependencies, as well as the JDK. 
This produces a self-contained native executable that only includes code that is actually necessary to build and execute a project. 
The result is a native image executable with high performance and less memory overhead, leading to smaller container images. 
This optimal resource consumption with less CPU and memory is ideal for the cloud, making Java applications easy to ship and deploy directly (such as in a microservices-based architecture).

% A paragraph describing the current limitations of GraalVM
The GraalVM native image technology relies on static analysis to build a native executable that only includes the elements reachable from an application entry point, its dependencies, and the JDK classes discovered.
To do so, the points-to analysis of the AOT compilation needs to “reach” all the bytecode to work correctly~\cite{wimmer2021graalvm}. 
This means that all the bytecode in the application and their dependencies that can be called at runtime must be known at build time (observed and analyzed), \ie, when the native-image tool in GraalVM is building the standalone executable.
This limitation is known as the \emph{closed-world assumption}~\cite{Wimmer2019}. 
The reachability of some elements (such as classes, methods, or fields) may not be discoverable due to the Java dynamic features, \eg, reflection, resource access, dynamic proxies, and serialization~\cite{sui2018soundness, landman2017challenges,li2019understanding, reif2019judge}.
Consequently, dynamic language capabilities such as Java Native Interface (JNI), Java Reflection, Dynamic Proxy objects (\texttt{java.lang.reflect.Proxy}), or classpath resources (\texttt{Class.getResource}) are not supported.
The closed-world constraint imposes strict limits on the natural dynamism of Java, particularly on the run-time reflection and class-loading features upon which so many existing libraries and frameworks depend. 
For the time being, not all applications are well suited to this constraint, and not all developers are willing to live with it.

% A paragraph about the need to use a gradual incremental approach to port the dependencies that are affected by the limitations
If an element is not reachable, it is not included in the generated executable and this can lead to runtime failures. 
To include elements whose reachability is undiscoverable, the native image builder requires externally provided reachability metadata.
To mitigate this limitation, GraalVM provides a tracing Java agent that tracks all usages of dynamic features utilized by a running JVM.
This agent interfaces with the JVM at runtime and intercepts all calls that look up classes, methods, fields, resources, or request proxy accesses. 
The agent then writes a report with all the intercepted dynamic accesses. 
This report can be passed to the native-image tool so that the used classes will not be removed during the image build process.

Therefore, rather than adopt the closed-world constraint at the start, the Java community instead pursues a gradual, incremental approach.
Today the community works incrementally along this spectrum of constraints, starting small and simple in order to develop a firm understanding of the changes required to the Java Platform Specification. while preserving the core values of readability, compatibility, and generality. 
In the long run, Java will likely embrace the full closed-world constraint in order to produce fully-static images. 
Between now and then, however, the community works on developing and delivering incremental improvements which developers can use sooner rather than later.
A notable effort is the GraalVM Reachability Metadata Repository~\cite{GraalVMReachabilityMetadata2023}, which enables native image users to share and reuse metadata for libraries and frameworks in the Java ecosystem, and thus simplify the maintenance of third-party dependencies. 
The repository is integrated with GraalVM Native Build Tools beginning with version \texttt{0.9.13}, and integrates with notable Java web frameworks such as Spring Boot 3.0, Quarkus, and Micronaut~\cite{vsipek2020enhancing}.

% The future is with GraalVM, but meanwhile, we need DepTrim
GraalVM and native image compilation is perceived by many as the future of JVM-based languages.
However, since the native image creation process analyzes the bytecode in the application and all its dependencies, there is a risk of violating the close world if at least one of the dependencies relies on some dynamic Java feature. 
The community is creating new versions of libraries that respect this assumption. 
However, there is still insufficient support for the most popular Java libraries. 
This technology still needs some time to mature before its massive adoption.
In this paper, we introduce a novel technique to specialize the third-party dependencies of Java applications by removing unused classes. 
Our approach is unique in the sense that it takes into account the fact that many dependencies may violate the close world assumption.

==> old-text.tex <==
% \author{\IEEEauthorblockN{C\'esar Soto-Valero\IEEEauthorrefmark{1}, Deepika Tiwari\IEEEauthorrefmark{1}, and Benoit Baudry\IEEEauthorrefmark{1}}


First, for a project which can be deployed and executed directly as an application, end-users can exercise their specialized versions under production workloads.
Second, a specialized project that is intended to be used as a library can be declared as dependency within client projects.



% \IEEEauthorblockA{\IEEEauthorrefmark{1}\textit{KTH Royal Institute of Technology, Stockholm, Sweden}\\ Email: \{cesarsv, deepikat, baudry\}@kth.se\\}}

% \deptrim substitutes original libraries with diverse combinations of specialized library variants, resulting in a population of diversified client projects.

We analyze the similarities and differences among the Y variants produced by \deptrim. Furthermore, we find that the P\% of client test suites successfully execute with the variants. 
% synonym trim => prune

% to manage project build and dependencies
%in  the size of their total classes,
% that builds correctly with \mv (\ie, the project's source code and a corresponding \pom file).
% The project builds correctly with the specialized dependencies and the specialized \pom.  
% , \ie dependencies with at least one used class member 
iterates over the set of specialized dependencies and attempts to build the project with one specialized dependency at a time, while maintaining a record of the builds that were successful. Finally,
the union of all the successfully build dependency trees to produce
%that are successfully built, as well as the number of specialized dependencies that the project is built with.
% that handles the data collection and execution of \deptrim for our study subjects. 
%First, the original dependency tree is resolved and dependencies are fetched from an external repository to the local repository . 
% For the used dependencies that have at least one used class member, \deptrim proceeds to remove all the unused class files. 
% To do so, it iterates over the dependencies in the dependency tree of $\mathcal{P}$ (line \autoref{line:algo:specialization-iteration-one}). For each dependency, \deptrim identifies the classes within it that are reachable from $\mathcal{P}$, using the pre-computed static call graph $\mathcal{CG}$ (line \autoref{line:algo:specialization-reachable}). Next, \deptrim prepares a set of specialized dependencies of $\mathcal{P}$, each containing only the classes identified as reachable. 
% On line \autoref{line:algo:specialization-deploy}, \deptrim deploys these specialized dependencies to the local repository.
%Finally, the dependency tree specialization phase produces a version of the \pom that points to these specialized versions of the dependencies.
% Once the specialized dependencies are deployed in the local repository, 
%Next, individual dependencies are specialized through the removal of unused classes within them, based on the call graph analysis. 
%
%In the following subsections, we describe each phase in more detail. 

% \autoref{alg:specialization} details the subroutine corresponding to the dependency tree specialization (lines \autoref{line:algo:specialization-init} to \autoref{line:algo:specialization-end}).
% Based on the build results of the project, \deptrim will determine the extent of the dependencies' bytecode that is exercised by the project.
% Thus, it is likely that \deptrim will remove large swathes of the project’s \texttt{compile} scope dependencies.

% diversify the software supply chain through debloating. Specifically, we produce specialized variants of libraries that can be used within client projects that only invoke specific functionalities of these libraries.
This gives rise to the \emph{Software Supply Chain}.
This phenomenon, termed as the software supply chain, is evidence of the collaborative nature of software development.

Developers choose between multiple libraries that offer overlapping functionalities, as well as multiple versions of these libraries~

% Discuss the maven build system and the concept of dependencies
% The \maven ecosystem includes a vast repository of libraries tailored to solve specific problems. 
% Developers can easily import these libraries into their  projects, by declaring them as dependencies~\cite{SotoValero2019}. 
% By leveraging the functionalities offered by dependencies, developers can focus on building the unique features of their system.
% While this makes software development convenient, it also has downsides. 
% First, developers may declare a dependency without actually using it.
% Second, a dependency itself may have downstream, or \emph{transitive}, dependencies, which all get added to the project distributable. 
% In practice, it is common for developers only to use a small subset of the functionalities provided by dependencies, especially transitive ones. 
% This causes a significant amount of unnecessary code, or bloat, to be included in the project, increasing its size and attack surface~\cite{soto2021comprehensive}.

\begin{definition}
% of a \maven project includes the dependencies resolved by \maven 
%  In order to construct the dependency tree, \maven identifies direct dependencies based on the project \pom, 
% To construct the dependency tree, Maven relies on a specific dependency resolution mechanism~\cite{MavenDependencyMechanism2021}.

%\todo{@Deepika: Describe \autoref{tab:descriptive}. Refer to the concept of technical leverage~\cite{massacci2021technical} when describing the ratios. Also refer to Prazi~\cite{hejderup2022prazi}}
% The following is our contribution and should not be in the background IMO
% If all the dependencies in the dependency tree of a project are specialized such that the project still builds, the dependency tree is totally specialized dependencies. On the other hand, if only a subset of the dependencies can be specialized such that the project builds, the dependency tree is partially specialized.

% figure description
% \autoref{fig:descriptive-stats} summarizes descriptive statistics of the projects considered for the evaluation of \deptrim. 
% The projects are well-known in the Java community.
% \autoref{fig:descriptive-stats-commits} shows the distribution of number of Git commits (1st Qu. = \np{1268}, Median = \np{2544}, 3rd Qu. = \np{5156}). The project with the largest number of commits is \texttt{flink} with \np{32667} commits.
% \autoref{fig:descriptive-stats-stars} shows the distribution of the number of stars on GitHub (1st Qu. = \np{1864}, Median = \np{2751}, 3rd Qu. = \np{4392}). The projects with the highest and lowest number of stars are \texttt{commons-validator} (\np{155}) and \texttt{flink} (\np{20488}), respectively.
% \autoref{fig:descriptive-stats-loc} shows the distribution of the number of lines of Java code (LoC), computed by the Unix command \texttt{cloc} (1st Qu. = \np{16531}, Median = \np{32965}, 3rd Qu. = \np{65052}). The two projects with the largest LoC are \texttt{CoreNLP} (\np{605561}) and \texttt{checkstyle} (\np{342795}).
% \autoref{fig:descriptive-stats-loc} shows the distribution of the number of tests executed by the official \texttt{maven-surefire-plugin} in the projects (1st Qu. = \np{132}, Median = \np{599}, 3rd Qu. = \np{952}). The four projects with the most tests are \texttt{jimfs} (\np{5834}), \texttt{checkstyle} (\np{3887}), \texttt{lettuce} (\np{2600}), and \texttt{graphhopper} (\np{2460}).


\textbf{Direct dependencies: }\normalfont
The set of dependencies of a \maven project that are declared in its \pom file are called direct dependencies. A direct dependency is added to the \pom by the developers, who explicitly manifest the intention of using the dependency.
% example
For example, in \autoref{fig:jacop-dt-original}, \texttt{scala-library} is one of the \np{6} direct dependencies of \texttt{jacop} because it is specified in the \pom of \jacop.
\end{definition}

\begin{definition}
\textbf{Transitive dependencies: }\normalfont
The set of transitive dependencies of a \maven project includes the dependencies resolved by \maven from the transitive closure of direct dependencies. 
Transitive dependencies are resolved automatically by \maven, which means that developers do not need to explicitly declare these dependencies.
% example
In addition to the \np{6} direct dependencies of \jacop, as illustrated in \autoref{fig:jacop-dt-original}, it has \np{5} transitive ones. \texttt{scala-reflect} is a dependency of \texttt{scala-compiler}, which makes it a transitive dependency of \jacop.
\end{definition}

% The authors queried the GitHub API on June 9th of 2020, to find all the projects that use Java as the primary programming language
% there is no free lunch regarding the addition of dependencies because their presence creates

In order to answer RQ1, we invoke \deptrim on each project in the dataset, as described in \autoref{sec:tool}. This means that each project is debloated and its dependencies specialized, based on their usage. \deptrim then attempts to build the project, \ie, compile it and run its tests, with the largest subset of specialized dependencies. This subset is selected through the following protocol. First, \deptrim tries to build the project with all dependencies specialized (TST). If the build is successful, \deptrim returns this TST. However, if the build is unsuccessful, \deptrim iterates over the set of specialized dependencies and attempts to build the project with one specialized dependency at a time (SST), while maintaining a record of the builds that were successful. Finally, \deptrim computes the union of all the successful SSTs to produce a PST, which has the largest subset of specialized dependencies using which the project still successfully builds. \deptrim returns this PST. We report the number of projects that are successfully built, as well as the number of specialized dependencies that the project is built with.


% background
A software system relies on the functionalities offered by a multitude of other systems, or libraries, to achieve its use cases. This phenomenon, termed as the software supply chain, is evidence of the collaborative nature of software development.
% problem
However, the libraries that a software system depends on are rarely used in their entirety, resulting in bloat and a potentially larger attack surface.
% solution
In this paper, we present \deptrim, a tool that specializes a library based on its usage by a client. \deptrim systematically identifies the subset of functionalities of a library that are required by the client, and trims the rest. The output is a debloated variant of the library, that can substitute the original one within the client.
% evaluation
We evaluate \deptrim with X Java libraries published on Maven Central, that are used by thousands of clients. \deptrim specializes the X libraries to produce a total Y variants for Z distinct clients.
% results
We analyze the similarities and differences among the Y variants produced by \deptrim. Furthermore, we find that the P\% of client test suites successfully execute with the variants. Our results imply that diversification within the open-source software supply chain is achievable through library specialization.

\newcommand{\RQone}{How many unique library versions do we generate?\xspace}
\newcommand{\RQtwo}{How many clients can diversify their supply chain?\xspace} 
\newcommand{\RQthree}{How many clients behave correctly with diverse supply chains?\xspace}



\begin{figure}[t]
    \centering
  \subfloat[\#Commits\label{fig:descriptive-stats-commits}]{%
        \includegraphics[width=0.22\linewidth]{figures/commits.pdf}}
        \hfill
  \subfloat[\#Stars\label{fig:descriptive-stats-stars}]{%
       \includegraphics[width=0.22\linewidth]{figures/stars.pdf}}
       \hfill
  \subfloat[\#LoC\label{fig:descriptive-stats-loc}]{%
        \includegraphics[width=0.22\linewidth]{figures/loc.pdf}}
        \hfill
  \subfloat[\#Tests\label{fig:descriptive-stats-tests}]{%
        \includegraphics[width=0.22\linewidth]{figures/tests.pdf}}
        \hfill
  \caption{Descriptive statistics of the \np{30} projects used for the evaluation of \deptrim. Average values are marked with $\times$.}
  \label{fig:descriptive-stats} 
\end{figure}

% RW old
Their analysis is fine-grained down to the level of methods and fields, to preserve behaviors after removing unnecessary bytecode.
%A prototype of \libcapsule has been developed and evaluated with a dataset of 204 popular third-party libraries and 2,021 apps. Results indicate that it is able to enforce complete and fine-grained regulation on third-party libraries according to customized security policies with a low performance overhead.
% Their approach involves symbolically executing source programs in conjunction with calls to a partial evaluator.
The specialized programs are synthesized
% They ensure its correctness through the use of a bisimulation relation on the source and specialized programs.

% para one: specialized projects are being used by users directly or by client projects. how do we validate the runtime behaviour beyond the test suite?

% There are two possible solutions: we either curate a set of clients for each specialized projects, such that the clients have test suites that actually exercise the specialized project (a.k.a Reverse dependency compatibility testing \cite{ochoa2022breakbot}). The alternative is to use the cli of the specialized project with a production workload.

% para three: We take the second approach and use the cli of three projects in our dataset - recap these projects, explain protocol (workload), and results. Discuss implications.

% the project's build with a specialized dependency fails due to compilation errors or test failures. \todo{@Deepika: Update this caption. Note: ratio in RQ1 is nbcd classes / project classes, sometimes \depclean removes bloated dependencies with 0 classes - they are resources / avoid conflicts, etc}


==> tables/depclean.tex <==
\begin{table}
\centering
\scriptsize
\caption{Dependency debloating with \depclean (baseline).}
\label{tab:depclean}
\begin{tabular}{|l|r|r|r|} 
\hline
\multirow{2}{*}{\textsc{Project}}                    & \multicolumn{3}{c|}{\textsc{Non-Bloated Compile Scope Dependencies}}                                                    \\ 
\cline{2-4}
                                                     & \multicolumn{1}{c|}{\textsc{Used}} & \multicolumn{1}{c|}{\textsc{\#Classes}} & \multicolumn{1}{c|}{\textsc{Size (KB)}}  \\ 
\hline
\rowcolor[rgb]{0.961,0.961,0.961} checkstyle         & \ChartSmall[r]{15}{17}             & \np{6491}                               & \np{14070}                               \\
Chronicle-Map                                        & \ChartSmall[r]{24}{35}             & \np{7087}                               & \np{14987}                               \\
\rowcolor[rgb]{0.961,0.961,0.961} classgraph         & \ChartSmall[r]{2}{2}               & \np{224}                                & \np{334}                                 \\
commons-validator                                    & \ChartSmall[r]{4}{4}               & \np{780}                                & \np{1067}                                \\
\rowcolor[rgb]{0.961,0.961,0.961} CoreNLP            & \ChartSmall[r]{29}{32}             & \np{8685}                               & \np{16230}                               \\
flink                                                & \ChartSmall[r]{14}{16}             & \np{6173}                               & \np{9749}                                \\
\rowcolor[rgb]{0.961,0.961,0.961} graphhopper\_core  & \ChartSmall[r]{13}{18}             & \np{4165}                               & \np{9704}                                \\
guice                                                & \ChartSmall[r]{7}{10}              & \np{2466}                               & \np{3175}                                \\
\rowcolor[rgb]{0.961,0.961,0.961} helidon-io/openapi & \ChartSmall[r]{33}{36}             & \np{3951}                               & \np{6798}                                \\
httpcomponents-client                                & \ChartSmall[r]{4}{5}               & \np{1134}                               & \np{5625}                                \\
\rowcolor[rgb]{0.961,0.961,0.961} immutables/gson    & \ChartSmall[r]{2}{2}               & \np{307}                                & \np{346}                                 \\
jacop                                                & \ChartSmall[r]{4}{9}               & \np{7983}                               & \np{21666}                               \\
\rowcolor[rgb]{0.961,0.961,0.961} java-faker         & \ChartSmall[r]{4}{4}               & \np{506}                                & \np{951}                                 \\
jcabi-github                                         & \ChartSmall[r]{16}{20}             & \np{3912}                               & \np{8542}                                \\
\rowcolor[rgb]{0.961,0.961,0.961} jooby              & \ChartSmall[r]{20}{22}             & \np{6945}                               & \np{11529}                               \\
jimfs                                                & \ChartSmall[r]{6}{9}               & \np{3557}                               & \np{15679}                               \\
\rowcolor[rgb]{0.961,0.961,0.961} lettuce/core       & \ChartSmall[r]{37}{44}             & \np{10327}                              & \np{15862}                               \\
modelmapper                                          & \ChartSmall[r]{5}{6}               & \np{2692}                               & \np{3795}                                \\
\rowcolor[rgb]{0.961,0.961,0.961} mybatis-3          & \ChartSmall[r]{8}{8}               & \np{1345}                               & \np{2197}                                \\
OpenPDF                                              & \ChartSmall[r]{12}{35}             & \np{15176}                              & \np{39242}                               \\
\rowcolor[rgb]{0.961,0.961,0.961} pdfbox             & \ChartSmall[r]{6}{7}               & \np{6773}                               & \np{14428}                               \\
pf4j                                                 & \ChartSmall[r]{2}{3}               & \np{72}                                 & \np{203}                                 \\
\rowcolor[rgb]{0.961,0.961,0.961} poi-tl             & \ChartSmall[r]{28}{36}             & \np{11743}                              & \np{22280}                               \\
Recaf                                                & \ChartSmall[r]{41}{56}             & \np{9902}                               & \np{19805}                               \\
\rowcolor[rgb]{0.961,0.961,0.961} scribejava         & \ChartSmall[r]{6}{8}               & \np{1238}                               & \np{2594}                                \\
RxRelay                                              & \ChartSmall[r]{2}{2}               & \np{1758}                               & \np{2585}                                \\
\rowcolor[rgb]{0.961,0.961,0.961} tablesaw           & \ChartSmall[r]{7}{9}               & \np{1352}                               & \np{2831}                                \\
tika                                                 & \ChartSmall[r]{2}{2}               & \np{253}                                & \np{378}                                 \\
\rowcolor[rgb]{0.961,0.961,0.961} undertow           & \ChartSmall[r]{5}{5}               & \np{742}                                & \np{1154}                                \\
woodstox                                             & \ChartSmall[r]{5}{5}               & \np{864}                                & \np{1179}                                \\ 
\hline
\textsc{Total}                                       & \ChartSmall[r]{364}{467}           & \np{128603}                             & \np{268985}                              \\
\hline
\end{tabular}
\end{table}

==> tables/deptrim.tex <==
% \cellcolor[HTML]{FCFFEB}
\begin{table*}
\footnotesize
\centering
% https://www.color-hex.com/color-palette/1021912
\caption{Results from the evaluation of \deptrim with the case studies described in \autoref{tab:descriptive}. For RQ1, the table indicates the number of non-bloated \compile-scope dependencies (\nbcd). These are the dependencies that are identified as used in the project by \depclean. The number of classes removed via debloating is listed in the column \textsc{Classes Removed}.
\ratiod represents the number of remaining third-party classes after debloating over the number of classes in the project.
For RQ2, we highlight whether \deptrim builds a project with a \tst or a \pst, as well as the number of specialized NBCDs contained in the built project (\textsc{NBCD Specialized}).
RQ3 presents the reduction in the number of classes in the NBCDs as a result of specialization with \deptrim, and correspondingly, in the \ratios of the third-party classes to project classes.
For RQ4, we report the three cases where specialization with \deptrim is not applicable: (i) if all the classes in a non-bloated dependency are totally used by the project (\tud); (ii) if specializing a dependency causes a compilation error (\textsc{Comp. Error}) during project build; and (iii) if a test fails when building a project with a specialized dependency (\textsc{Test Fail.}). \textcolor{white}{\href{https://github.com/DiUS/java-faker/blob/master/src/main/resources/en/hitchhikers\_guide\_to\_the\_galaxy.yml\#L41}{DON'T PANIC}}}

% the project's build with a specialized dependency fails due to compilation errors or test failures. \todo{@Deepika: Update this caption. Note: ratio in RQ1 is nbcd classes / project classes, sometimes \depclean removes bloated dependencies with 0 classes - they are resources / avoid conflicts, etc}
\label{tab:deptrim}
\setlength\tabcolsep{2pt}
\begin{tabular}{|l||r|r|r||c|c|r||r|r||r|r|r|} 
\hline
\multirow{3}{*}{\textsc{Project}}                     & \multicolumn{3}{c||}{{\cellcolor[rgb]{0.961,0.957,0.996}}RQ1}                                                                                                                                                                                                     & \multicolumn{3}{c||}{{\cellcolor[rgb]{0.988,0.996,0.922}}RQ2}                                                                                                                                                              & \multicolumn{2}{c||}{{\cellcolor[rgb]{0.886,0.992,0.988}}RQ3}                                                                                                          & \multicolumn{3}{c|}{{\cellcolor[rgb]{0.882,1,0.882}}RQ4}                                                                                                                                                                        \\ 
\hhline{|~||---||---||--||---|}
                                                      & \multicolumn{1}{c|}{{\cellcolor[rgb]{0.961,0.957,0.996}}}                                & \multicolumn{1}{c|}{{\cellcolor[rgb]{0.961,0.957,0.996}}\textsc{Classes}} & \multicolumn{1}{c||}{{\cellcolor[rgb]{0.961,0.957,0.996}}}                                 & {\cellcolor[rgb]{0.988,0.996,0.922}}                                & {\cellcolor[rgb]{0.988,0.996,0.922}}                                & \multicolumn{1}{c||}{{\cellcolor[rgb]{0.988,0.996,0.922}}\textsc{NBCD}}        & \multicolumn{1}{c|}{{\cellcolor[rgb]{0.886,0.992,0.988}}\textsc{Classes}} & \multicolumn{1}{c||}{{\cellcolor[rgb]{0.886,0.992,0.988}}}                                 & \multicolumn{1}{c|}{{\cellcolor[rgb]{0.882,1,0.882}}}                               & \multicolumn{1}{c|}{{\cellcolor[rgb]{0.882,1,0.882}}\textsc{Comp.}} & \multicolumn{1}{c|}{{\cellcolor[rgb]{0.882,1,0.882}}\textsc{Test}}  \\
                                                      & \multicolumn{1}{c|}{\multirow{-2}{*}{{\cellcolor[rgb]{0.961,0.957,0.996}}\textsc{NBCD}}} & \multicolumn{1}{c|}{{\cellcolor[rgb]{0.961,0.957,0.996}}\textsc{Removed}} & \multicolumn{1}{c||}{\multirow{-2}{*}{{\cellcolor[rgb]{0.961,0.957,0.996}}\ratiod}} & \multirow{-2}{*}{{\cellcolor[rgb]{0.988,0.996,0.922}}\textsc{\tst}} & \multirow{-2}{*}{{\cellcolor[rgb]{0.988,0.996,0.922}}\textsc{\pst}} & \multicolumn{1}{c||}{{\cellcolor[rgb]{0.988,0.996,0.922}}\textsc{Specialized}} & \multicolumn{1}{c|}{{\cellcolor[rgb]{0.886,0.992,0.988}}\textsc{Removed}} & \multicolumn{1}{c||}{\multirow{-2}{*}{{\cellcolor[rgb]{0.886,0.992,0.988}}\ratios}} & \multicolumn{1}{c|}{\multirow{-2}{*}{{\cellcolor[rgb]{0.882,1,0.882}}\textsc{TUD}}} & \multicolumn{1}{c|}{{\cellcolor[rgb]{0.882,1,0.882}}\textsc{Error}} & \multicolumn{1}{c|}{{\cellcolor[rgb]{0.882,1,0.882}}\textsc{Fail.}}  \\ 
\hline
\rowcolor[rgb]{0.91,0.918,0.918} \texttt{checkstyle}  & \np{15}/\np{17}                                                                          & \ChartSmall[p]{2}{6493}                                                   & \Ratio{863}{6491}                                                                          & \textcolor{red}{\ding{55}}                                          & \textcolor{teal}{\ding{51}}                                         & \np{12}/\np{15}                                                                & \ChartSmall[p]{2330}{6491}                                                & \Ratio{863}{4161}                                                                          & \np{0}/\np{15}                                                                      & \np{2}/\np{3}                                                       & \np{1}/\np{3}                                                       \\
\texttt{Chronicle-Map}                                & {\cellcolor[rgb]{0.996,1,1}}\np{28}/\np{35}                                              & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{278}{7595}                     & {\cellcolor[rgb]{0.996,1,1}}\Ratio{375}{7317}                                              & {\cellcolor[rgb]{0.996,1,1}}\textcolor{red}{\ding{55}}              & {\cellcolor[rgb]{0.996,1,1}}\textcolor{teal}{\ding{51}}             & {\cellcolor[rgb]{0.996,1,1}}\np{22}/\np{28}                                    & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{4670}{7317}                    & {\cellcolor[rgb]{0.996,1,1}}\Ratio{375}{2647}                                              & {\cellcolor[rgb]{0.996,1,1}}\np{4}/\np{28}                                          & {\cellcolor[rgb]{0.996,1,1}}\np{1}/\np{2}                           & {\cellcolor[rgb]{0.996,1,1}}\np{1}/\np{2}                           \\
\rowcolor[rgb]{0.91,0.918,0.918} \texttt{classgraph}  & \np{2}/\np{2}                                                                            & \ChartSmall[p]{0}{224}                                                    & \Ratio{261}{224}                                                                           & \textcolor{teal}{\ding{51}}                                         &                                                                     & \np{2}/\np{2}                                                                  & \ChartSmall[p]{10}{224}                                                   & \Ratio{261}{214}                                                                           & \np{0}/\np{2}                                                                       & --                                                                  & --                                                                  \\
\texttt{commons-validator}                            & {\cellcolor[rgb]{0.996,1,1}}\np{4}/\np{4}                                                & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{0}{780}                        & {\cellcolor[rgb]{0.996,1,1}}\Ratio{64}{780}                                                & {\cellcolor[rgb]{0.996,1,1}}\textcolor{teal}{\ding{51}}             & {\cellcolor[rgb]{0.996,1,1}}                                        & {\cellcolor[rgb]{0.996,1,1}}\np{4}/\np{4}                                      & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{625}{780}                      & {\cellcolor[rgb]{0.996,1,1}}\Ratio{64}{155}                                                & {\cellcolor[rgb]{0.996,1,1}}\np{0}/\np{4}                                           & {\cellcolor[rgb]{0.996,1,1}}--                                      & {\cellcolor[rgb]{0.996,1,1}}--                                      \\
\rowcolor[rgb]{0.91,0.918,0.918} \texttt{CoreNLP}     & \np{30}/\np{32}                                                                          & \ChartSmall[p]{364}{9121}                                                 & \Ratio{3932}{8757}                                                                         & \textcolor{teal}{\ding{51}}                                         &                                                                     & \np{29}/\np{30}                                                                & \ChartSmall[p]{3648}{8757}                                                & \Ratio{3932}{5109}                                                                         & \np{1}/\np{30}                                                                      & --                                                                  & --                                                                  \\
\texttt{flink}                                        & {\cellcolor[rgb]{0.996,1,1}}\np{15}/\np{16}                                              & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{0}{6175}                       & {\cellcolor[rgb]{0.996,1,1}}\Ratio{277}{6175}                                              & {\cellcolor[rgb]{0.996,1,1}}\textcolor{red}{\ding{55}}              & {\cellcolor[rgb]{0.996,1,1}}\textcolor{teal}{\ding{51}}             & {\cellcolor[rgb]{0.996,1,1}}\np{12}/\np{15}                                    & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{4124}{6175}                    & {\cellcolor[rgb]{0.996,1,1}}\Ratio{277}{2051}                                              & {\cellcolor[rgb]{0.996,1,1}}\np{1}/\np{15}                                          & {\cellcolor[rgb]{0.996,1,1}}\np{1}/\np{2}                           & {\cellcolor[rgb]{0.996,1,1}}\np{1}/\np{2}                           \\
\rowcolor[rgb]{0.91,0.918,0.918} \texttt{graphhopper} & \np{13}/\np{18}                                                                          & \ChartSmall[p]{1309}{5474}                                                & \Ratio{631}{4165}                                                                          & \textcolor{red}{\ding{55}}                                          & \textcolor{teal}{\ding{51}}                                         & \np{12}/\np{13}                                                                & \ChartSmall[p]{1666}{4165}                                                & \Ratio{631}{2499}                                                                          & \np{0}/\np{13}                                                                      & \np{1}/\np{1}                                                       & \np{0}/\np{1}                                                       \\
\texttt{guice}                                        & {\cellcolor[rgb]{0.996,1,1}}\np{9}/\np{10}                                               & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{0}{2474}                       & {\cellcolor[rgb]{0.996,1,1}}\Ratio{460}{2474}                                              & {\cellcolor[rgb]{0.996,1,1}}\textcolor{teal}{\ding{51}}             & {\cellcolor[rgb]{0.996,1,1}}                                        & {\cellcolor[rgb]{0.996,1,1}}\np{7}/\np{9}                                      & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{1327}{2474}                    & {\cellcolor[rgb]{0.996,1,1}}\Ratio{460}{1147}                                              & {\cellcolor[rgb]{0.996,1,1}}\np{2}/\np{9}                                           & {\cellcolor[rgb]{0.996,1,1}}--                                      & {\cellcolor[rgb]{0.996,1,1}}--                                      \\
\rowcolor[rgb]{0.91,0.918,0.918} \texttt{helidon-io}  & \np{34}/\np{36}                                                                          & \ChartSmall[p]{38}{4002}                                                  & \Ratio{32}{3964}                                                                           & \textcolor{red}{\ding{55}}                                          & \textcolor{teal}{\ding{51}}                                         & \np{32}/\np{34}                                                                & \ChartSmall[p]{1040}{3964}                                                & \Ratio{32}{2924}                                                                           & \np{1}/\np{34}                                                                      & \np{1}/\np{1}                                                       & \np{0}/\np{1}                                                       \\
\texttt{httpcomponents-client}                        & {\cellcolor[rgb]{0.996,1,1}}\np{5}/\np{5}                                                & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{0}{1153}                       & {\cellcolor[rgb]{0.996,1,1}}\Ratio{493}{1153}                                              & {\cellcolor[rgb]{0.996,1,1}}\textcolor{teal}{\ding{51}}             & {\cellcolor[rgb]{0.996,1,1}}                                        & {\cellcolor[rgb]{0.996,1,1}}\np{4}/\np{5}                                      & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{432}{1153}                     & {\cellcolor[rgb]{0.996,1,1}}\Ratio{493}{721}                                               & {\cellcolor[rgb]{0.996,1,1}}\np{1}/\np{5}                                           & {\cellcolor[rgb]{0.996,1,1}}--                                      & {\cellcolor[rgb]{0.996,1,1}}--                                      \\
\rowcolor[rgb]{0.91,0.918,0.918} \texttt{immutables}  & \np{2}/\np{2}                                                                            & \ChartSmall[p]{0}{307}                                                    & \Ratio{31}{307}                                                                            & \textcolor{teal}{\ding{51}}                                         &                                                                     & \np{2}/\np{2}                                                                  & \ChartSmall[p]{48}{307}                                                   & \Ratio{31}{259}                                                                            & \np{0}/\np{2}                                                                       & --                                                                  & --                                                                  \\
\texttt{jacop}                                        & {\cellcolor[rgb]{0.996,1,1}}\np{4}/\np{9}                                                & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{504}{8487}                     & {\cellcolor[rgb]{0.996,1,1}}\Ratio{833}{7983}                                              & {\cellcolor[rgb]{0.996,1,1}}\textcolor{red}{\ding{55}}              & {\cellcolor[rgb]{0.996,1,1}}\textcolor{teal}{\ding{51}}             & {\cellcolor[rgb]{0.996,1,1}}\np{3}/\np{4}                                      & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{6453}{7983}                    & {\cellcolor[rgb]{0.996,1,1}}\Ratio{833}{1530}                                              & {\cellcolor[rgb]{0.996,1,1}}\np{0}/\np{4}                                           & {\cellcolor[rgb]{0.996,1,1}}\np{1}/\np{1}                           & {\cellcolor[rgb]{0.996,1,1}}\np{0}/\np{1}                           \\
\rowcolor[rgb]{0.91,0.918,0.918} \texttt{java-faker}  & \np{4}/\np{4}                                                                            & \ChartSmall[p]{0}{506}                                                    & \Ratio{107}{506}                                                                           & \textcolor{red}{\ding{55}}                                          & \textcolor{teal}{\ding{51}}                                         & \np{3}/\np{4}                                                                  & \ChartSmall[p]{222}{506}                                                  & \Ratio{107}{284}                                                                           & \np{0}/\np{4}                                                                       & \np{1}/\np{1}                                                       & \np{0}/\np{1}                                                       \\
\texttt{jcabi-github}                                 & {\cellcolor[rgb]{0.996,1,1}}\np{17}/\np{20}                                              & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{9}{3921}                       & {\cellcolor[rgb]{0.996,1,1}}\Ratio{312}{3912}                                              & {\cellcolor[rgb]{0.996,1,1}}\textcolor{red}{\ding{55}}              & {\cellcolor[rgb]{0.996,1,1}}\textcolor{teal}{\ding{51}}             & {\cellcolor[rgb]{0.996,1,1}}\np{16}/\np{17}                                    & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{2456}{3912}                    & {\cellcolor[rgb]{0.996,1,1}}\Ratio{312}{1456}                                              & {\cellcolor[rgb]{0.996,1,1}}\np{0}/\np{17}                                          & {\cellcolor[rgb]{0.996,1,1}}\np{1}/\np{1}                           & {\cellcolor[rgb]{0.996,1,1}}\np{0}/\np{1}                           \\
\rowcolor[rgb]{0.91,0.918,0.918} \texttt{jimfs}       & \np{8}/\np{9}                                                                            & \ChartSmall[p]{0}{3560}                                                   & \Ratio{124}{3560}                                                                          & \textcolor{teal}{\ding{51}}                                         &                                                                     & \np{6}/\np{8}                                                                  & \ChartSmall[p]{1741}{3560}                                                & \Ratio{124}{1819}                                                                          & \np{2}/\np{8}                                                                       & --                                                                  & --                                                                  \\
\texttt{jooby}                                        & {\cellcolor[rgb]{0.996,1,1}}\np{20}/\np{22}                                              & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{0}{6945}                       & {\cellcolor[rgb]{0.996,1,1}}\Ratio{320}{6945}                                              & {\cellcolor[rgb]{0.996,1,1}}\textcolor{red}{\ding{55}}              & {\cellcolor[rgb]{0.996,1,1}}\textcolor{teal}{\ding{51}}             & {\cellcolor[rgb]{0.996,1,1}}\np{19}/\np{20}                                    & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{1349}{6945}                    & {\cellcolor[rgb]{0.996,1,1}}\Ratio{320}{5596}                                              & {\cellcolor[rgb]{0.996,1,1}}\np{0}/\np{20}                                          & {\cellcolor[rgb]{0.996,1,1}}\np{1}/\np{1}                           & {\cellcolor[rgb]{0.996,1,1}}\np{0}/\np{1}                           \\
\rowcolor[rgb]{0.91,0.918,0.918} \texttt{lettuce}     & \np{39}/\np{44}                                                                          & \ChartSmall[p]{0}{10364}                                                  & \Ratio{1302}{10364}                                                                        & \textcolor{red}{\ding{55}}                                          & \textcolor{teal}{\ding{51}}                                         & \np{36}/\np{39}                                                                & \ChartSmall[p]{1866}{10364}                                               & \Ratio{1302}{8498}                                                                         & \np{2}/\np{39}                                                                      & \np{0}/\np{1}                                                       & \np{1}/\np{1}                                                       \\
\texttt{modelmapper}                                  & {\cellcolor[rgb]{0.996,1,1}}\np{6}/\np{6}                                                & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{0}{2700}                       & {\cellcolor[rgb]{0.996,1,1}}\Ratio{210}{2700}                                              & {\cellcolor[rgb]{0.996,1,1}}\textcolor{red}{\ding{55}}              & {\cellcolor[rgb]{0.996,1,1}}\textcolor{teal}{\ding{51}}             & {\cellcolor[rgb]{0.996,1,1}}\np{4}/\np{6}                                      & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{412}{2700}                     & {\cellcolor[rgb]{0.996,1,1}}\Ratio{210}{2288}                                              & {\cellcolor[rgb]{0.996,1,1}}\np{1}/\np{6}                                           & {\cellcolor[rgb]{0.996,1,1}}\np{0}/\np{1}                           & {\cellcolor[rgb]{0.996,1,1}}\np{1}/\np{1}                           \\
\rowcolor[rgb]{0.91,0.918,0.918} \texttt{mybatis-3}   & \np{8}/\np{8}                                                                            & \ChartSmall[p]{0}{1345}                                                   & \Ratio{480}{1345}                                                                          & \textcolor{red}{\ding{55}}                                          & \textcolor{teal}{\ding{51}}                                         & \np{7}/\np{8}                                                                  & \ChartSmall[p]{422}{1345}                                                 & \Ratio{480}{923}                                                                           & \np{0}/\np{8}                                                                       & \np{0}/\np{1}                                                       & \np{1}/\np{1}                                                       \\
\texttt{OpenPDF}                                      & {\cellcolor[rgb]{0.996,1,1}}\np{12}/\np{35}                                              & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{2336}{17512}                   & {\cellcolor[rgb]{0.996,1,1}}\Ratio{484}{15176}                                             & {\cellcolor[rgb]{0.996,1,1}}\textcolor{red}{\ding{55}}              & {\cellcolor[rgb]{0.996,1,1}}\textcolor{teal}{\ding{51}}             & {\cellcolor[rgb]{0.996,1,1}}\np{11}/\np{12}                                    & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{11468}{15176}                  & {\cellcolor[rgb]{0.996,1,1}}\Ratio{484}{3708}                                              & {\cellcolor[rgb]{0.996,1,1}}\np{0}/\np{12}                                          & {\cellcolor[rgb]{0.996,1,1}}\np{1}/\np{1}                           & {\cellcolor[rgb]{0.996,1,1}}\np{0}/\np{1}                           \\
\rowcolor[rgb]{0.91,0.918,0.918} \texttt{pdfbox}      & \np{6}/\np{7}                                                                            & \ChartSmall[p]{63}{6836}                                                  & \Ratio{754}{6773}                                                                          & \textcolor{teal}{\ding{51}}                                         &                                                                     & \np{6}/\np{6}                                                                  & \ChartSmall[p]{5070}{6773}                                                & \Ratio{754}{1703}                                                                          & \np{0}/\np{6}                                                                       & --                                                                  & --                                                                  \\
\texttt{pf4j}                                         & {\cellcolor[rgb]{0.996,1,1}}\np{3}/\np{3}                                                & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{0}{115}                        & {\cellcolor[rgb]{0.996,1,1}}\Ratio{93}{115}                                                & {\cellcolor[rgb]{0.996,1,1}}\textcolor{teal}{\ding{51}}             & {\cellcolor[rgb]{0.996,1,1}}                                        & {\cellcolor[rgb]{0.996,1,1}}\np{2}/\np{3}                                      & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{10}{115}                       & {\cellcolor[rgb]{0.996,1,1}}\Ratio{93}{105}                                                & {\cellcolor[rgb]{0.996,1,1}}\np{1}/\np{3}                                           & {\cellcolor[rgb]{0.996,1,1}}--                                      & {\cellcolor[rgb]{0.996,1,1}}--                                      \\
\rowcolor[rgb]{0.91,0.918,0.918} \texttt{poi-tl}      & \np{33}/\np{36}                                                                          & \ChartSmall[p]{258}{12143}                                                & \Ratio{255}{11885}                                                                         & \textcolor{red}{\ding{55}}                                          & \textcolor{teal}{\ding{51}}                                         & \np{27}/\np{33}                                                                & \ChartSmall[p]{5192}{11885}                                               & \Ratio{255}{6693}                                                                          & \np{5}/\np{33}                                                                      & \np{0}/\np{1}                                                       & \np{1}/\np{1}                                                       \\
\texttt{Recaf}                                        & {\cellcolor[rgb]{0.996,1,1}}\np{49}/\np{56}                                              & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{518}{10769}                    & {\cellcolor[rgb]{0.996,1,1}}\Ratio{538}{10251}                                             & {\cellcolor[rgb]{0.996,1,1}}\textcolor{teal}{\ding{51}}             & {\cellcolor[rgb]{0.996,1,1}}                                        & {\cellcolor[rgb]{0.996,1,1}}\np{41}/\np{49}                                    & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{2952}{10251}                   & {\cellcolor[rgb]{0.996,1,1}}\Ratio{538}{7299}                                              & {\cellcolor[rgb]{0.996,1,1}}\np{8}/\np{49}                                          & {\cellcolor[rgb]{0.996,1,1}}--                                      & {\cellcolor[rgb]{0.996,1,1}}--                                      \\
\rowcolor[rgb]{0.91,0.918,0.918} \texttt{RxRelay}     & \np{2}/\np{2}                                                                            & \ChartSmall[p]{0}{1758}                                                   & \Ratio{16}{1758}                                                                           & \textcolor{red}{\ding{55}}                                          & \textcolor{teal}{\ding{51}}                                         & \np{1}/\np{2}                                                                  & \ChartSmall[p]{64}{1758}                                                  & \Ratio{16}{1694}                                                                           & \np{0}/\np{2}                                                                       & \np{0}/\np{1}                                                       & \np{1}/\np{1}                                                       \\
\texttt{scribejava}                                   & {\cellcolor[rgb]{0.996,1,1}}\np{7}/\np{8}                                                & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{39}{1278}                      & {\cellcolor[rgb]{0.996,1,1}}\Ratio{116}{1239}                                              & {\cellcolor[rgb]{0.996,1,1}}\textcolor{teal}{\ding{51}}             & {\cellcolor[rgb]{0.996,1,1}}                                        & {\cellcolor[rgb]{0.996,1,1}}\np{6}/\np{7}                                      & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{353}{1239}                     & {\cellcolor[rgb]{0.996,1,1}}\Ratio{116}{886}                                               & {\cellcolor[rgb]{0.996,1,1}}\np{1}/\np{7}                                           & {\cellcolor[rgb]{0.996,1,1}}--                                      & {\cellcolor[rgb]{0.996,1,1}}--                                      \\
\rowcolor[rgb]{0.91,0.918,0.918} \texttt{tablesaw}    & \np{9}/\np{9}                                                                            & \ChartSmall[p]{0}{1447}                                                   & \Ratio{7}{1447}                                                                            & \textcolor{teal}{\ding{51}}                                         &                                                                     & \np{7}/\np{9}                                                                  & \ChartSmall[p]{379}{1447}                                                 & \Ratio{7}{1068}                                                                            & \np{2}/\np{9}                                                                       & --                                                                  & --                                                                  \\
\texttt{tika}                                         & {\cellcolor[rgb]{0.996,1,1}}\np{2}/\np{2}                                                & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{0}{253}                        & {\cellcolor[rgb]{0.996,1,1}}\Ratio{435}{253}                                               & {\cellcolor[rgb]{0.996,1,1}}\textcolor{teal}{\ding{51}}             & {\cellcolor[rgb]{0.996,1,1}}                                        & {\cellcolor[rgb]{0.996,1,1}}\np{2}/\np{2}                                      & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{187}{253}                      & {\cellcolor[rgb]{0.996,1,1}}\Ratio{435}{66}                                                & {\cellcolor[rgb]{0.996,1,1}}\np{0}/\np{2}                                           & {\cellcolor[rgb]{0.996,1,1}}--                                      & {\cellcolor[rgb]{0.996,1,1}}--                                      \\
\rowcolor[rgb]{0.91,0.918,0.918} \texttt{undertow}    & \np{5}/\np{5}                                                                            & \ChartSmall[p]{0}{742}                                                    & \Ratio{1581}{742}                                                                          & \textcolor{teal}{\ding{51}}                                         &                                                                     & \np{5}/\np{5}                                                                  & \ChartSmall[p]{224}{742}                                                  & \Ratio{1581}{518}                                                                          & \np{0}/\np{5}                                                                       & --                                                                  & --                                                                  \\
\texttt{woodstox}                                     & {\cellcolor[rgb]{0.996,1,1}}\np{5}/\np{5}                                                & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{0}{864}                        & {\cellcolor[rgb]{0.996,1,1}}\Ratio{208}{864}                                               & {\cellcolor[rgb]{0.996,1,1}}\textcolor{red}{\ding{55}}              & {\cellcolor[rgb]{0.996,1,1}}\textcolor{teal}{\ding{51}}             & {\cellcolor[rgb]{0.996,1,1}}\np{3}/\np{5}                                      & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{222}{864}                      & {\cellcolor[rgb]{0.996,1,1}}\Ratio{208}{642}                                               & {\cellcolor[rgb]{0.996,1,1}}\np{0}/\np{5}                                           & {\cellcolor[rgb]{0.996,1,1}}\np{1}/\np{2}                           & {\cellcolor[rgb]{0.996,1,1}}\np{1}/\np{2}                           \\ 
\hline
\textsc{Total}                                        & {\cellcolor[rgb]{0.996,1,1}}\np{396}/\np{467}                                            & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{5718}{135343}                  & {\cellcolor[rgb]{0.996,1,1}}\Ratio{15594}{129625}                                          & \multicolumn{1}{r|}{{\cellcolor[rgb]{0.996,1,1}}\np{14}/\np{30}}    & \multicolumn{1}{r|}{{\cellcolor[rgb]{0.996,1,1}}\np{16}/\np{30}}    & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{343}{396}                           & {\cellcolor[rgb]{0.996,1,1}}\ChartSmall[p]{60962}{129625}                 & {\cellcolor[rgb]{0.996,1,1}}\Ratio{15594}{68663}                                           & {\cellcolor[rgb]{0.996,1,1}}\np{32}/\np{396}                                        & {\cellcolor[rgb]{0.996,1,1}}\np{12}/\np{21}                         & {\cellcolor[rgb]{0.996,1,1}}\np{9}/\np{21}                          \\
\hline
\end{tabular}
% \vspace{0.25cm}
\end{table*}


==> tables/descriptive.tex <==
\begin{table*}
\centering
\footnotesize
\caption{Description of the study subjects considered for the evaluation of \deptrim. The table links to the project repository and SHA on GitHub, and lists the number of commits, stars, lines of Java code (LoC), tests, and the original number of \texttt{compile}-scope dependencies in the project (\#\cd). Also indicated are the number of project classes in each study subject, the total number of classes contributed by {\cd}s, as well as the ratio between them (\ratioo). 
\textcolor{white}{\texttt{the cake is a lie}}}
%\caption{Ratio of number of classes and project binaries \wrt non-bloated compile scope dependencies (NBCD).}
\label{tab:descriptive}
\setlength\tabcolsep{3pt}
\begin{tabular}{|l|c|c|r|r|r|r|r|r|r|r|} 
\hline
\multirow{2}{*}{\textsc{Project}}                                                                                    & \multirow{2}{*}{\textsc{Module}} & \multirow{2}{*}{\textsc{Commit SHA}}                                                                                                                 & \multicolumn{1}{c|}{\multirow{2}{*}{\textsc{Commits}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textsc{Stars}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textsc{LoC}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textsc{Tests}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textsc{\#CD}}} & \multicolumn{3}{c|}{\textsc{Classes}}                                                                                               \\ 
\cline{9-11}
                                                                                                                                           &                                  &                                                                                                                                                      & \multicolumn{1}{c|}{}                                    & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{}                                & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{\textsc{Project}}  & \multicolumn{1}{c|}{\textsc{CD}}        & \multicolumn{1}{c|}{\ratioo}                \\ 
\hline
\rowcolor[rgb]{0.91,0.918,0.918} 
\href{https://github.com/checkstyle/checkstyle}{\texttt{checkstyle}}                                           & \texttt{--}                      & \texttt{\href{https://github.com/checkstyle/checkstyle/commit/dbeb9024c861ad11b194e40d8c6e08d7e6ec5122}{6ec5122}}        & \np{12066}                   & \np{7455}                  & \np{342795}              & \np{3887}                  & \np{17}                 & \np{863}   & \np{6493}   & \Ratio{863}{6493}      \\
\href{https://github.com/OpenHFT/Chronicle-Map}{\texttt{Chronicle-Map}}                                        & \texttt{--}                      & \texttt{\href{https://github.com/OpenHFT/Chronicle-Map/commit/26e26c132290ad8049c97e0c44eb7f33b63c1c60}{63c1c60}}        & \np{3298}                    & \np{2539}                  & \np{55178}               & \np{1231}                  & \np{35}                 & \np{375}   & \np{7595}   & \Ratio{375}{7595}      \\
\rowcolor[rgb]{0.91,0.918,0.918} 
\href{https://github.com/classgraph/classgraph}{\texttt{classgraph}}                                           & \texttt{--}                      & \texttt{\href{https://github.com/classgraph/classgraph/commit/92b644677964496fb841ba41bed52247f8a24786}{8a24786}}        & \np{5307}                    & \np{2366}                  & \np{32151}               & \np{170}                   & \np{2}                  & \np{261}   & \np{224}    & \Ratio{261}{224}       \\
\href{https://github.com/apache/commons-validator}{\texttt{commons-validator}}                                 & \texttt{--}                      & \texttt{\href{https://github.com/apache/commons-validator/commit/f9bb21748a9f9c50fbc31862de25ed49433ecc88}{33ecc88}}     & \np{1742}                    & \np{155}                   & \np{16781}               & \np{576}                   & \np{4}                  & \np{64}    & \np{780}    & \Ratio{64}{780}        \\
\rowcolor[rgb]{0.91,0.918,0.918} 
\href{https://github.com/stanfordnlp/CoreNLP}{\texttt{CoreNLP}}                                                & \texttt{--}                      & \texttt{\href{https://github.com/checkstyle/checkstyle/commit/f7782ff5f235584b0fc559f266961b5ab013556a}{013556a}}        & \np{17012}                   & \np{8802}                  & \np{605561}              & \np{1374}                  & \np{32}                 & \np{3932}  & \np{9121}   & \Ratio{3932}{9121}     \\
\href{https://github.com/apache/flink}{\texttt{flink}}                                                         & \texttt{flink-java}              & \texttt{\href{https://github.com/apache/flink/commit/c41c8e5cfab683da8135d6c822693ef851d6e2b7}{1d6e2b7}}                 & \np{32667}                   & \np{20488}                 & \np{36455}               & \np{836}                   & \np{16}                 & \np{277}   & \np{6175}   & \Ratio{277}{6175}      \\
\rowcolor[rgb]{0.91,0.918,0.918} 
\href{https://github.com/graphhopper/graphhopper}{\texttt{graphhopper}}                                        & \texttt{core}                    & \texttt{\href{https://github.com/graphhopper/graphhopper/commit/6d3da37960f56aa6b9c4b1ffd77f70ebebff8747}{bff8747}}      & \np{6211}                    & \np{3978}                  & \np{66119}               & \np{2460}                  & \np{18}                 & \np{631}   & \np{5474}   & \Ratio{631}{5474}      \\
\href{https://github.com/google/guice}{\texttt{guice}}                                                         & \texttt{core}                    & \texttt{\href{https://github.com/google/guice/commit/b0ff10c8ec8911137451623a333d6daa65f73d8a}{5f73d8a}}                 & \np{2026}                    & \np{11730}                 & \np{49697}               & \np{979}                   & \np{10}                 & \np{460}   & \np{2474}   & \Ratio{460}{2474}      \\
\rowcolor[rgb]{0.91,0.918,0.918} 
\href{https://github.com/helidon-io/helidon}{\texttt{helidon-io}}                                              & \texttt{openapi}                 & \texttt{\href{https://github.com/helidon-io/helidon/commit/99cf5add9b4049581f08aae9eddaf0280070f2bb}{070f2bb}}           & \np{2707}                    & \np{2929}                  & \np{7729}                & \np{30}                    & \np{36}                 & \np{32}    & \np{4002}   & \Ratio{32}{4002}       \\
\href{https://github.com/apache/httpcomponents-client/tree/master/httpclient5}{\texttt{httpcomponents-client}} & \texttt{httpclient5}             & \texttt{\href{https://github.com/apache/httpcomponents-client/commit/d8f702fb4d44c746bb0edf00643aa7139cb8bdf7}{cb8bdf7}} & \np{3424}                    & \np{1269}                  & \np{42920}               & \np{669}                   & \np{5}                  & \np{493}   & \np{1153}   & \Ratio{493}{1153}      \\
\rowcolor[rgb]{0.91,0.918,0.918} 
\href{https://github.com/immutables/immutables}{\texttt{immutables}}                                           & \texttt{gson}                    & \texttt{\href{https://github.com/immutables/immutables/commit/6e192030320eaf7a8b5f146c39ae5a17b413aa37}{413aa37}}        & \np{2588}                    & \np{3218}                  & \np{16448}               & \np{37}                    & \np{2}                  & \np{31}    & \np{307}    & \Ratio{31}{307}        \\
\href{https://github.com/radsz/jacop}{\texttt{jacop}}                                                          & \texttt{--}                      & \texttt{\href{https://github.com/radsz/jacop/commit/1a395e6add22caf79590fe9d1b2223bfb6ed0cd0}{6ed0cd0}}                  & \np{1302}                    & \np{202}                   & \np{93170}               & \np{210}                   & \np{9}                  & \np{833}   & \np{8487}   & \Ratio{833}{8487}      \\
\rowcolor[rgb]{0.91,0.918,0.918} 
\href{https://github.com/DiUS/java-faker}{\texttt{java-faker}}                                                 & \texttt{--}                      & \texttt{\href{https://github.com/DiUS/java-faker/commit/e23d6067c8f83b335a037d24e6107a37eb0b9e6e}{b0b9e6e}}              & \np{834}                     & \np{3914}                  & \np{8429}                & \np{579}                   & \np{4}                  & \np{107}   & \np{503}    & \Ratio{107}{503}       \\
\href{https://github.com/jcabi/jcabi-github}{\texttt{jcabi-github}}                                            & \texttt{--}                      & \texttt{\href{https://github.com/jcabi/jcabi-github/commit/02f3ab93156349c2f66989ac675bd6292462d724}{462d724}}           & \np{2764}                    & \np{276}                   & \np{33542}               & \np{684}                   & \np{20}                 & \np{312}   & \np{3921}   & \Ratio{312}{3921}      \\
\rowcolor[rgb]{0.91,0.918,0.918} 
\href{https://github.com/google/jimfs}{\texttt{jimfs}}                                                         & \texttt{jimfs}                   & \texttt{\href{https://github.com/google/jimfs/commit/3bc54fae2feb218dcf5427d2626720fc09ef38d1}{9ef38d1}}                 & \np{508}                     & \np{2234}                  & \np{15558}               & \np{5834}                  & \np{9}                  & \np{124}   & \np{3560}   & \Ratio{124}{3560}      \\
\href{https://github.com/jooby-project/jooby/tree/3.x/jooby}{\texttt{jooby}}                                   & \texttt{jooby}                   & \texttt{\href{https://github.com/jooby-project/jooby/commit/4d7be54dad429b5aeb5266387df14b0781c78357}{1c78357}}          & \np{4702}                    & \np{1523}                  & \np{20154}               & \np{122}                   & \np{22}                 & \np{320}   & \np{6945}   & \Ratio{320}{6945}      \\
\rowcolor[rgb]{0.91,0.918,0.918} 
\href{https://github.com/lettuce-io/lettuce-core}{\texttt{lettuce}}                                            & \texttt{core}                    & \texttt{\href{https://github.com/lettuce-io/lettuce-core/commit/77c4ea587fdba73f688c95a481d2743b6fc94fcb}{fc94fcb}}      & \np{2280}                    & \np{4861}                  & \np{89468}               & \np{2600}                  & \np{44}                 & \np{1302}  & \np{10364}  & \Ratio{1302}{10364}    \\
\href{https://github.com/modelmapper/modelmapper}{\texttt{modelmapper}}                                        & \texttt{core}                    & \texttt{\href{https://github.com/modelmapper/modelmapper/commit/894c658609f47f817ce20e41f6e87e1f803663ee}{03663ee}}      & \np{721}                     & \np{2090}                  & \np{21769}               & \np{618}                   & \np{6}                  & \np{210}   & \np{2700}   & \Ratio{210}{2700}      \\
\rowcolor[rgb]{0.91,0.918,0.918} 
\href{https://github.com/mybatis/mybatis-3}{\texttt{mybatis-3}}                                                & \texttt{--}                      & \texttt{\href{https://github.com/mybatis/mybatis-3/commit/c195f12808a88a1ee245dc86d9c1621042655970}{2655970}}            & \np{4436}                    & \np{18065}                 & \np{61849}               & \np{1699}                  & \np{8}                  & \np{480}   & \np{1345}   & \Ratio{480}{1345}      \\
\href{https://github.com/LibrePDF/OpenPDF}{\texttt{OpenPDF}}                                                   & \texttt{--}                      & \texttt{\href{https://github.com/LibrePDF/OpenPDF/commit/0c9c4ca393b01444b7cb13bb1d12da202bd0d458}{bd0d458}}             & \np{1296}                    & \np{2573}                  & \np{76397}               & \np{35}                    & \np{35}                 & \np{484}   & \np{17512}  & \Ratio{484}{17512}     \\
\rowcolor[rgb]{0.91,0.918,0.918} 
\href{https://github.com/apache/pdfbox/tree/trunk/pdfbox}{\texttt{pdfbox}}                                     & \texttt{pdfbox}                  & \texttt{\href{https://github.com/apache/pdfbox/commit/e72963ca5b283a87828ee731cd85c0b6baf1ff57}{af1ff57}}                & \np{11147}                   & \np{1852}                  & \np{97175}               & \np{654}                   & \np{7}                  & \np{754}   & \np{6836}   & \Ratio{754}{6836}      \\
\href{https://github.com/pf4j/pf4j}{\texttt{pf4j}}                                                             & \texttt{--}                      & \texttt{\href{https://github.com/pf4j/pf4j/commit/efaed93c10dd9d114335e2a344e8bca04fd00c63}{fd00c63}}                    & \np{692}                     & \np{1901}                  & \np{7199}                & \np{151}                   & \np{3}                  & \np{93}    & \np{115}    & \Ratio{93}{115}        \\
\rowcolor[rgb]{0.91,0.918,0.918} 
\href{https://github.com/Sayi/poi-tl}{\texttt{poi-tl}}                                                         & \texttt{--}                      & \texttt{\href{https://github.com/Sayi/poi-tl/commit/5d5004311a406b7d5843be76322bf208071b5969}{71b5969}}                  & \np{732}                     & \np{3063}                  & \np{20882}               & \np{125}                   & \np{36}                 & \np{255}   & \np{12143}  & \Ratio{255}{12143}     \\
\href{https://github.com/Col-E/Recaf}{\texttt{Recaf}}                                                          & \texttt{--}                      & \texttt{\href{https://github.com/Col-E/Recaf/commit/c66f23801493bd866db757b0594c1fceaa30dce0}{a30dce0}}                  & \np{2275}                    & \np{4530}                  & \np{31277}               & \np{274}                   & \np{56}                 & \np{538}   & \np{10769}  & \Ratio{538}{10769}     \\
\rowcolor[rgb]{0.91,0.918,0.918} 
\href{https://github.com/JakeWharton/RxRelay}{\texttt{RxRelay}}                                                & \texttt{--}                      & \texttt{\href{https://github.com/JakeWharton/RxRelay/commit/e9fc1586192ca1ecdbc41ae39036cbf0d09428b5}{09428b5}}          & \np{81}                      & \np{2473}                  & \np{2405}                & \np{64}                    & \np{2}                  & \np{16}    & \np{1758}   & \Ratio{16}{1758}       \\
\href{https://github.com/scribejava/scribejava}{\texttt{scribejava}}                                           & \texttt{--}                      & \texttt{\href{https://github.com/scribejava/commit/466f37c6faf5a9a2de9c87ae1bce71b617a6185b}{7a6185b}}                   & \np{1259}                    & \np{5317}                  & \np{5769}                & \np{82}                    & \np{8}                  & \np{116}   & \np{1278}   & \Ratio{116}{1278}      \\
\rowcolor[rgb]{0.91,0.918,0.918} 
\href{https://github.com/jtablesaw/tablesaw/tree/master/json}{\texttt{tablesaw}}                               & \texttt{json}                    & \texttt{\href{https://github.com/jtablesaw/tablesaw/commit/05823f66246ea191e62ad0658d2fed0b080d5334}{80d5334}}           & \np{2501}                    & \np{3101}                  & \np{508}                 & \np{9}                     & \np{9}                  & \np{7}     & \np{1447}   & \Ratio{7}{1447}        \\
\href{https://github.com/apache/tika/tree/main/tika-core}{\texttt{tika}}                                       & \texttt{tika-core}               & \texttt{\href{https://github.com/apache/tika/commit/41319f3c294b13de5342a80570b4540f7dd04a3e}{dd04a3e}}                  & \np{6823}                    & \np{1584}                  & \np{32388}               & \np{305}                   & \np{2}                  & \np{435}   & \np{253}    & \Ratio{435}{253}       \\
\rowcolor[rgb]{0.91,0.918,0.918} 
\href{https://github.com/undertow-io/undertow/tree/master/core}{\texttt{undertow}}                             & \texttt{core}                    & \texttt{\href{https://github.com/undertow-io/undertow/commit/56c91f129b1c2a55cf3287836cc68c80acce54c6}{cce54c6}}         & \np{5517}                    & \np{3284}                  & \np{106711}              & \np{682}                   & \np{5}                  & \np{1581}  & \np{742}    & \Ratio{1581}{742}      \\
\href{https://github.com/FasterXML/woodstox}{\texttt{woodstox}}                                                & \texttt{--}                      & \texttt{\href{https://github.com/FasterXML/woodstox/commit/e8f00401bebd103f62d51383ef53da2cd58bd89e}{58bd89e}}           & \np{325}                     & \np{180}                   & \np{60476}               & \np{868}                   & \np{5}                  & \np{208}   & \np{864}    & \Ratio{208}{864}       \\
\hline
\textsc{Total}                                                                                                 & \np{14}                          & \np{30}                                                                                                                  & \np{139243}                  & \np{127952}                & \np{2056960}             & \np{27844}                 & \np{467}                & \np{15594} & \np{135343} & \Ratio{15594}{135343}  \\
\hline
\end{tabular}
\end{table*}

% https://youtu.be/dQw4w9WgXcQ

==> tests_failures_logs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%
% poi-tl
%%%%%%%%%%%%%%%%%%%%%%%%%

[INFO]  T E S T S
[INFO] -------------------------------------------------------
[INFO] Running com.deepoove.poi.tl.config.ElementTemplateFactoryTest
[ERROR] Tests run: 1, Failures: 0, Errors: 1, Skipped: 0, Time elapsed: 0.453 s <<< FAILURE! - in com.deepoove.poi.tl.config.ElementTemplateFactoryTest
[ERROR] testConfigRenderDataCompute  Time elapsed: 0.432 s  <<< ERROR!
java.lang.NoSuchMethodError: 'byte[] org.apache.commons.io.IOUtils.byteArray(int)'
	at com.deepoove.poi.tl.config.ElementTemplateFactoryTest.testConfigRenderDataCompute(ElementTemplateFactoryTest.java:42)

 
[INFO] Running com.deepoove.poi.tl.plugin.SectionTableRenderPolicyTest
[ERROR] Tests run: 1, Failures: 0, Errors: 1, Skipped: 0, Time elapsed: 0.001 s <<< FAILURE! - in com.deepoove.poi.tl.plugin.SectionTableRenderPolicyTest
[ERROR] test  Time elapsed: 0 s  <<< ERROR!
java.lang.NoSuchMethodError: 'byte[] org.apache.commons.io.IOUtils.byteArray(int)'
	at com.deepoove.poi.tl.plugin.SectionTableRenderPolicyTest.test(SectionTableRenderPolicyTest.java:28)

[INFO] Running com.deepoove.poi.tl.plugin.HackLoopTableRenderPolicyTest
[ERROR] Tests run: 1, Failures: 0, Errors: 1, Skipped: 0, Time elapsed: 0 s <<< FAILURE! - in com.deepoove.poi.tl.plugin.HackLoopTableRenderPolicyTest
[ERROR] testPaymentHackExample  Time elapsed: 0 s  <<< ERROR!
java.lang.NoSuchMethodError: 'byte[] org.apache.commons.io.IOUtils.byteArray(int)'
	at com.deepoove.poi.tl.plugin.HackLoopTableRenderPolicyTest.testPaymentHackExample(HackLoopTableRenderPolicyTest.java:65)

[INFO] Running com.deepoove.poi.tl.plugin.PaginationRenderPolicyTest
[ERROR] Tests run: 1, Failures: 0, Errors: 1, Skipped: 0, Time elapsed: 0 s <<< FAILURE! - in com.deepoove.poi.tl.plugin.PaginationRenderPolicyTest
[ERROR] testPagination  Time elapsed: 0 s  <<< ERROR!
java.lang.NoSuchMethodError: 'byte[] org.apache.commons.io.IOUtils.byteArray(int)'
	at com.deepoove.poi.tl.plugin.PaginationRenderPolicyTest.testPagination(PaginationRenderPolicyTest.java:22)

[INFO] Running com.deepoove.poi.tl.plugin.MultipleRowTableRenderPolicyTest
[ERROR] Tests run: 1, Failures: 0, Errors: 1, Skipped: 0, Time elapsed: 0 s <<< FAILURE! - in com.deepoove.poi.tl.plugin.MultipleRowTableRenderPolicyTest
[ERROR] testMultiRow  Time elapsed: 0 s  <<< ERROR!
java.lang.NoSuchMethodError: 'byte[] org.apache.commons.io.IOUtils.byteArray(int)'
	at com.deepoove.poi.tl.plugin.MultipleRowTableRenderPolicyTest.testMultiRow(MultipleRowTableRenderPolicyTest.java:34)


%%%%%%%%%%%%%%%%%%%%%%%%%
% lettuce-core
%%%%%%%%%%%%%%%%%%%%%%%%%

[ERROR] io.lettuce.core.metrics.MicrometerCommandLatencyRecorderUnitTests.tags  Time elapsed: 0 s  <<< ERROR!
java.lang.NoClassDefFoundError: io/micrometer/core/instrument/simple/SimpleConfig
	at io.micrometer.core.instrument.simple.SimpleMeterRegistry.<init>(SimpleMeterRegistry.java:48)
	at io.lettuce.core.metrics.MicrometerCommandLatencyRecorderUnitTests.<init>(MicrometerCommandLatencyRecorderUnitTests.java:51)
	at java.base/jdk.internal.reflect.NativeConstructorAccessorImpl.newInstance0(Native Method)
	at java.base/jdk.internal.reflect.NativeConstructorAccessorImpl.newInstance(NativeConstructorAccessorImpl.java:62)
	at java.base/jdk.internal.reflect.DelegatingConstructorAccessorImpl.newInstance(DelegatingConstructorAccessorImpl.java:45)
	at java.base/java.lang.reflect.Constructor.newInstance(Constructor.java:490)
	at org.junit.platform.commons.util.ReflectionUtils.newInstance(ReflectionUtils.java:552)
	at org.junit.jupiter.engine.execution.ConstructorInvocation.proceed(ConstructorInvocation.java:56)



%%%%%%%%%%%%%%%%%%%%%%%%%
% RxRelay
%%%%%%%%%%%%%%%%%%%%%%%%%

 Results :

Tests in error: 
  ReplayRelayTest.reentrantDrain:467 NoClassDefFound io/reactivex/rxjava3/schedu...
  ReplayRelayTest.takeSizeAndTime:436 NoClassDefFound io/reactivex/rxjava3/sched...
  ReplayRelayTest.testReplayTimestampedDirectly:98 NoClassDefFound io/reactivex/...
  ReplayRelayTest.testSizeAndHasAnyValueTimeBounded:189 NoClassDefFound io/react...
  ReplayRelayTest.timeAndSizeRemoveCorrectNumberOfOld:553 NoClassDefFound io/rea...
  ReplayRelayTest.timedSkipOld:422 NoClassDefFound io/reactivex/rxjava3/schedule...

Tests run: 64, Failures: 0, Errors: 6, Skipped: 3

[INFO] ------------------------------------------------------------------------
[INFO] BUILD FAILURE
[INFO] ------------------------------------------------------------------------


%%%%%%%%%%%%%%%%%%%%%%%%%
% Chronicle-map
%%%%%%%%%%%%%%%%%%%%%%%%%
[INFO] Tests run: 1, Failures: 0, Errors: 0, Skipped: 0, Time elapsed: 0.002 s - in net.openhft.chronicle.map.DatasetTrackerIssue61Test
[INFO] Running net.openhft.chronicle.map.channel.MapHandlerTest
[ERROR] Tests run: 5, Failures: 0, Errors: 3, Skipped: 2, Time elapsed: 1.514 s <<< FAILURE! - in net.openhft.chronicle.map.channel.MapHandlerTest
[ERROR] net.openhft.chronicle.map.channel.MapHandlerTest.passThroughMapFF  Time elapsed: 1.498 s  <<< ERROR!
net.openhft.chronicle.core.io.ClosedIORuntimeException: Closed
	at net.openhft.chronicle.wire.channel.impl.TCPChronicleChannel.readingDocument0(TCPChronicleChannel.java:207)
	at net.openhft.chronicle.wire.channel.impl.TCPChronicleChannel.readingDocument(TCPChronicleChannel.java:162)
	at net.openhft.chronicle.wire.VanillaMethodReader.readOne0(VanillaMethodReader.java:520)
	at net.openhft.chronicle.wire.VanillaMethodReader.readOne(VanillaMethodReader.java:516)
	at net.openhft.chronicle.map.channel.MapHandlerTest.doPassThroughMap(MapHandlerTest.java:82)
	at net.openhft.chronicle.map.channel.MapHandlerTest.passThroughMapFF(MapHandlerTest.java:29)
	at java.base/jdk.internal.reflect.NativeMethodAccessorImpl.invoke0(Native Method)
	at java.base/jdk.internal.reflect.NativeMethodAccessorImpl.invoke(NativeMethodAccessorImpl.java:62)
	at java.base/jdk.internal.reflect.DelegatingMethodAccessorImpl.invoke(DelegatingMethodAccessorImpl.java:43)
	at java.base/java.lang.reflect.Method.invoke(Method.java:566)
	at org.junit.runners.model.FrameworkMethod$1.runReflectiveCall(FrameworkMethod.java:59)
	at org.junit.internal.runners.model.ReflectiveCallable.run(ReflectiveCallable.java:12)
	at org.junit.runners.model.FrameworkMethod.invokeExplosively(FrameworkMethod.java:56)
	at org.junit.internal.runners.statements.InvokeMethod.evaluate(InvokeMethod.java:17)
	at org.junit.runners.ParentRunner$3.evaluate(ParentRunner.java:306)
	at org.junit.runners.BlockJUnit4ClassRunner$1.evaluate(BlockJUnit4ClassRunner.java:100)
	at org.junit.runners.ParentRunner.runLeaf(ParentRunner.java:366)
	at org.junit.runners.BlockJUnit4ClassRunner.runChild(BlockJUnit4ClassRunner.java:103)
	at org.junit.runners.BlockJUnit4ClassRunner.runChild(BlockJUnit4ClassRunner.java:63)
	at org.junit.runners.ParentRunner$4.run(ParentRunner.java:331)
	at org.junit.runners.ParentRunner$1.schedule(ParentRunner.java:79)
	at org.junit.runners.ParentRunner.runChildren(ParentRunner.java:329)
	at org.junit.runners.ParentRunner.access$100(ParentRunner.java:66)
	at org.junit.runners.ParentRunner$2.evaluate(ParentRunner.java:293)
	at org.junit.runners.ParentRunner$3.evaluate(ParentRunner.java:306)
	at org.junit.runners.ParentRunner.run(ParentRunner.java:413)
	at org.apache.maven.surefire.junit4.JUnit4Provider.execute(JUnit4Provider.java:377)
	at org.apache.maven.surefire.junit4.JUnit4Provider.executeWithRerun(JUnit4Provider.java:284)
	at org.apache.maven.surefire.junit4.JUnit4Provider.executeTestSet(JUnit4Provider.java:248)
	at org.apache.maven.surefire.junit4.JUnit4Provider.invoke(JUnit4Provider.java:167)
	at org.apache.maven.surefire.booter.ForkedBooter.runSuitesInProcess(ForkedBooter.java:456)
	at org.apache.maven.surefire.booter.ForkedBooter.execute(ForkedBooter.java:169)
	at org.apache.maven.surefire.booter.ForkedBooter.run(ForkedBooter.java:595)
	at org.apache.maven.surefire.booter.ForkedBooter.main(ForkedBooter.java:581)

[INFO] Results:
[INFO] 
[ERROR] Errors: 
[ERROR]   MapHandlerTest.passThroughMapFF:29->doPassThroughMap:82 » ClosedIORuntime Closed
[ERROR]   MapHandlerTest.passThroughMapFT:34->doPassThroughMap:82 » ClosedIORuntime Closed
[ERROR]   MapHandlerTest.passThroughServiceYaml:138 » NoClassDefFound net/openhft/chronicle/wire/TextMethodTester
[INFO] 
[ERROR] Tests run: 1231, Failures: 0, Errors: 3, Skipped: 19
[INFO] 
[INFO] ------------------------------------------------------------------------
[INFO] BUILD FAILURE
[INFO] ------------------------------------------------------------------------
[INFO] Total time:  08:04 min
[INFO] Finished at: 2023-01-21T14:01:40Z
[INFO] ------------------------------------------------------------------------






%%%%%%%%%%%%%%%%%%%%%%%%%
% Checkstyle
%%%%%%%%%%%%%%%%%%%%%%%%%

[ERROR] testMetadataFilesGenerationAllFiles{Capturable}  Time elapsed: 0.318 s  <<< ERROR!
java.lang.Error: Error was thrown while processing /Users/cesarsv/IdeaProjects/deptrim-experiments/pipeline/projects/checkstyle/src/main/java/com/puppycrawl/tools/checkstyle/checks/blocks/EmptyCatchBlockCheck.java
	at com.puppycrawl.tools.checkstyle.meta.MetadataGeneratorUtilTest.testMetadataFilesGenerationAllFiles(MetadataGeneratorUtilTest.java:75)
Caused by: javax.xml.transform.TransformerFactoryConfigurationError: Provider for class javax.xml.transform.TransformerFactory cannot be created
	at com.puppycrawl.tools.checkstyle.meta.MetadataGeneratorUtilTest.testMetadataFilesGenerationAllFiles(MetadataGeneratorUtilTest.java:75)
Caused by: java.lang.RuntimeException: Provider for class javax.xml.transform.TransformerFactory cannot be created
	at com.puppycrawl.tools.checkstyle.meta.MetadataGeneratorUtilTest.testMetadataFilesGenerationAllFiles(MetadataGeneratorUtilTest.java:75)
Caused by: java.util.ServiceConfigurationError: javax.xml.transform.TransformerFactory: Provider net.sf.saxon.TransformerFactoryImpl not found
	at com.puppycrawl.tools.checkstyle.meta.MetadataGeneratorUtilTest.testMetadataFilesGenerationAllFiles(MetadataGeneratorUtilTest.java:75)


%%%%%%%%%%%%%%%%%%%%%%%%%
% flink
%%%%%%%%%%%%%%%%%%%%%%%%%

[INFO] Running org.apache.flink.api.java.sampling.RandomSamplerTest
[ERROR] Tests run: 1, Failures: 0, Errors: 1, Skipped: 0, Time elapsed: 0.013 s <<< FAILURE! - in org.apache.flink.api.java.sampling.RandomSamplerTest
[ERROR] org.apache.flink.api.java.sampling.RandomSamplerTest  Time elapsed: 0.013 s  <<< ERROR!
java.lang.NoClassDefFoundError: org/apache/commons/math3/exception/TooManyIterationsException
	at org.apache.flink.api.java.sampling.RandomSamplerTest.<clinit>(RandomSamplerTest.java:65)
	at java.base/jdk.internal.reflect.NativeMethodAccessorImpl.invoke0(Native Method)
	at java.base/jdk.internal.reflect.NativeMethodAccessorImpl.invoke(NativeMethodAccessorImpl.java:62)
	at java.base/jdk.internal.reflect.DelegatingMethodAccessorImpl.invoke(DelegatingMethodAccessorImpl.java:43)
	at java.base/java.lang.reflect.Method.invoke(Method.java:566)
	at org.junit.runners.model.FrameworkMethod$1.runReflectiveCall(FrameworkMethod.java:59)
	at org.junit.internal.runners.model.ReflectiveCallable.run(ReflectiveCallable.java:12)
	at org.junit.runners.model.FrameworkMethod.invokeExplosively(FrameworkMethod.java:56)
	at org.junit.internal.runners.statements.RunBefores.invokeMethod(RunBefores.java:33)
	at org.junit.internal.runners.statements.RunBefores.evaluate(RunBefores.java:24)
	at org.junit.runners.ParentRunner$3.evaluate(ParentRunner.java:306)
	at org.junit.runners.ParentRunner.run(ParentRunner.java:413)
	at org.junit.runner.JUnitCore.run(JUnitCore.java:137)
	at org.junit.runner.JUnitCore.run(JUnitCore.java:115)
	at org.junit.vintage.engine.execution.RunnerExecutor.execute(RunnerExecutor.java:42)
	at org.junit.vintage.engine.VintageTestEngine.executeAllChildren(VintageTestEngine.java:80)
	at org.junit.vintage.engine.VintageTestEngine.execute(VintageTestEngine.java:72)
	at org.junit.platform.launcher.core.EngineExecutionOrchestrator.execute(EngineExecutionOrchestrator.java:107)
	at org.junit.platform.launcher.core.EngineExecutionOrchestrator.execute(EngineExecutionOrchestrator.java:88)
	at org.junit.platform.launcher.core.EngineExecutionOrchestrator.lambda$execute$0(EngineExecutionOrchestrator.java:54)
	at org.junit.platform.launcher.core.EngineExecutionOrchestrator.withInterceptedStreams(EngineExecutionOrchestrator.java:67)
	at org.junit.platform.launcher.core.EngineExecutionOrchestrator.execute(EngineExecutionOrchestrator.java:52)
	at org.junit.platform.launcher.core.DefaultLauncher.execute(DefaultLauncher.java:114)
	at org.junit.platform.launcher.core.DefaultLauncher.execute(DefaultLauncher.java:86)
	at org.junit.platform.launcher.core.DefaultLauncherSession$DelegatingLauncher.execute(DefaultLauncherSession.java:86)
	at org.junit.platform.launcher.core.SessionPerRequestLauncher.execute(SessionPerRequestLauncher.java:53)
	at org.apache.maven.surefire.junitplatform.JUnitPlatformProvider.lambda$execute$1(JUnitPlatformProvider.java:199)
	at java.base/java.util.Iterator.forEachRemaining(Iterator.java:133)
	at org.apache.maven.surefire.junitplatform.JUnitPlatformProvider.execute(JUnitPlatformProvider.java:193)
	at org.apache.maven.surefire.junitplatform.JUnitPlatformProvider.invokeAllTests(JUnitPlatformProvider.java:154)
	at org.apache.maven.surefire.junitplatform.JUnitPlatformProvider.invoke(JUnitPlatformProvider.java:120)
	at org.apache.maven.surefire.booter.ForkedBooter.runSuitesInProcess(ForkedBooter.java:428)
	at org.apache.maven.surefire.booter.ForkedBooter.execute(ForkedBooter.java:162)
	at org.apache.maven.surefire.booter.ForkedBooter.run(ForkedBooter.java:562)
	at org.apache.maven.surefire.booter.ForkedBooter.main(ForkedBooter.java:548)
Caused by: java.lang.ClassNotFoundException: org.apache.commons.math3.exception.TooManyIterationsException
	at java.base/jdk.internal.loader.BuiltinClassLoader.loadClass(BuiltinClassLoader.java:581)
	at java.base/jdk.internal.loader.ClassLoaders$AppClassLoader.loadClass(ClassLoaders.java:178)
	at java.base/java.lang.ClassLoader.loadClass(ClassLoader.java:522)
	... 35 more

%%%%%%%%%%%%%%%%%%%%%%%%%
% flink
%%%%%%%%%%%%%%%%%%%%%%%%%

[INFO] Running org.apache.flink.api.java.sampling.RandomSamplerTest
[ERROR] Tests run: 1, Failures: 0, Errors: 1, Skipped: 0, Time elapsed: 0.013 s <<< FAILURE! - in org.apache.flink.api.java.sampling.RandomSamplerTest
[ERROR] org.apache.flink.api.java.sampling.RandomSamplerTest  Time elapsed: 0.013 s  <<< ERROR!
java.lang.NoClassDefFoundError: org/apache/commons/math3/exception/TooManyIterationsException
	at org.apache.flink.api.java.sampling.RandomSamplerTest.<clinit>(RandomSamplerTest.java:65)
	at java.base/jdk.internal.reflect.NativeMethodAccessorImpl.invoke0(Native Method)
	at java.base/jdk.internal.reflect.NativeMethodAccessorImpl.invoke(NativeMethodAccessorImpl.java:62)
	at java.base/jdk.internal.reflect.DelegatingMethodAccessorImpl.invoke(DelegatingMethodAccessorImpl.java:43)
	at java.base/java.lang.reflect.Method.invoke(Method.java:566)
	at org.junit.runners.model.FrameworkMethod$1.runReflectiveCall(FrameworkMethod.java:59)
	at org.junit.internal.runners.model.ReflectiveCallable.run(ReflectiveCallable.java:12)
	at org.junit.runners.model.FrameworkMethod.invokeExplosively(FrameworkMethod.java:56)
	at org.junit.internal.runners.statements.RunBefores.invokeMethod(RunBefores.java:33)
	at org.junit.internal.runners.statements.RunBefores.evaluate(RunBefores.java:24)
	at org.junit.runners.ParentRunner$3.evaluate(ParentRunner.java:306)
	at org.junit.runners.ParentRunner.run(ParentRunner.java:413)
	at org.junit.runner.JUnitCore.run(JUnitCore.java:137)
	at org.junit.runner.JUnitCore.run(JUnitCore.java:115)
	at org.junit.vintage.engine.execution.RunnerExecutor.execute(RunnerExecutor.java:42)
	at org.junit.vintage.engine.VintageTestEngine.executeAllChildren(VintageTestEngine.java:80)
	at org.junit.vintage.engine.VintageTestEngine.execute(VintageTestEngine.java:72)
	at org.junit.platform.launcher.core.EngineExecutionOrchestrator.execute(EngineExecutionOrchestrator.java:107)
	at org.junit.platform.launcher.core.EngineExecutionOrchestrator.execute(EngineExecutionOrchestrator.java:88)
	at org.junit.platform.launcher.core.EngineExecutionOrchestrator.lambda$execute$0(EngineExecutionOrchestrator.java:54)
	at org.junit.platform.launcher.core.EngineExecutionOrchestrator.withInterceptedStreams(EngineExecutionOrchestrator.java:67)
	at org.junit.platform.launcher.core.EngineExecutionOrchestrator.execute(EngineExecutionOrchestrator.java:52)
	at org.junit.platform.launcher.core.DefaultLauncher.execute(DefaultLauncher.java:114)
	at org.junit.platform.launcher.core.DefaultLauncher.execute(DefaultLauncher.java:86)
	at org.junit.platform.launcher.core.DefaultLauncherSession$DelegatingLauncher.execute(DefaultLauncherSession.java:86)
	at org.junit.platform.launcher.core.SessionPerRequestLauncher.execute(SessionPerRequestLauncher.java:53)
	at org.apache.maven.surefire.junitplatform.JUnitPlatformProvider.lambda$execute$1(JUnitPlatformProvider.java:199)
	at java.base/java.util.Iterator.forEachRemaining(Iterator.java:133)
	at org.apache.maven.surefire.junitplatform.JUnitPlatformProvider.execute(JUnitPlatformProvider.java:193)
	at org.apache.maven.surefire.junitplatform.JUnitPlatformProvider.invokeAllTests(JUnitPlatformProvider.java:154)
	at org.apache.maven.surefire.junitplatform.JUnitPlatformProvider.invoke(JUnitPlatformProvider.java:120)
	at org.apache.maven.surefire.booter.ForkedBooter.runSuitesInProcess(ForkedBooter.java:428)
	at org.apache.maven.surefire.booter.ForkedBooter.execute(ForkedBooter.java:162)
	at org.apache.maven.surefire.booter.ForkedBooter.run(ForkedBooter.java:562)
	at org.apache.maven.surefire.booter.ForkedBooter.main(ForkedBooter.java:548)
Caused by: java.lang.ClassNotFoundException: org.apache.commons.math3.exception.TooManyIterationsException
	at java.base/jdk.internal.loader.BuiltinClassLoader.loadClass(BuiltinClassLoader.java:581)
	at java.base/jdk.internal.loader.ClassLoaders$AppClassLoader.loadClass(ClassLoaders.java:178)
	at java.base/java.lang.ClassLoader.loadClass(ClassLoader.java:522)
	... 35 more




%%%%%%%%%%%%%%%%%%%%%%%%%
% woodstox
%%%%%%%%%%%%%%%%%%%%%%%%%


 [INFO] Results:
[INFO] 
[ERROR] Errors: 
[ERROR]   TestWsdlValidation.setUp:84 » NoClassDefFound com/sun/msv/reader/xmlschema/WSD...
[INFO] 
[ERROR] Tests run: 868, Failures: 0, Errors: 1, Skipped: 0
[INFO] 
[INFO] ------------------------------------------------------------------------
[INFO] BUILD FAILURE
[INFO] ------------------------------------------------------------------------
[INFO] Total time:  17.686 s
[INFO] Finished at: 2023-01-06T13:46:35+01:00



==> utils/abbrev.tex <==
\usetikzlibrary{calc}
\usetikzlibrary{decorations.pathmorphing}

\makeatletter

\newcommand{\defhighlighter}[3][]{%
  \tikzset{every highlighter/.style={color=#2, fill opacity=#3, #1}}%
}

\defhighlighter{yellow}{.5}

\newcommand{\highlight@DoHighlight}{
  \fill [ decoration = {random steps, amplitude=1pt, segment length=15pt}
        , outer sep = -15pt, inner sep = 0pt, decorate
        , every highlighter, this highlighter ]
        ($(begin highlight)+(0,8pt)$) rectangle ($(end highlight)+(0,-3pt)$) ;
}

\newcommand{\highlight@BeginHighlight}{
  \coordinate (begin highlight) at (0,0) ;
}

\newcommand{\highlight@EndHighlight}{
  \coordinate (end highlight) at (0,0) ;
}

\newdimen\highlight@previous
\newdimen\highlight@current

\DeclareRobustCommand*\highlight[1][]{%
  \tikzset{this highlighter/.style={#1}}%
  \SOUL@setup
  %
  \def\SOUL@preamble{%
    \begin{tikzpicture}[overlay, remember picture]
      \highlight@BeginHighlight
      \highlight@EndHighlight
    \end{tikzpicture}%
  }%
  %
  \def\SOUL@postamble{%
    \begin{tikzpicture}[overlay, remember picture]
      \highlight@EndHighlight
      \highlight@DoHighlight
    \end{tikzpicture}%
  }%
  %
  \def\SOUL@everyhyphen{%
    \discretionary{%
      \SOUL@setkern\SOUL@hyphkern
      \SOUL@sethyphenchar
      \tikz[overlay, remember picture] \highlight@EndHighlight ;%
    }{%
    }{%
      \SOUL@setkern\SOUL@charkern
    }%
  }%
  %
  \def\SOUL@everyexhyphen##1{%
    \SOUL@setkern\SOUL@hyphkern
    \hbox{##1}%
    \discretionary{%
      \tikz[overlay, remember picture] \highlight@EndHighlight ;%
    }{%
    }{%
      \SOUL@setkern\SOUL@charkern
    }%
  }%
  %
  \def\SOUL@everysyllable{%
    \begin{tikzpicture}[overlay, remember picture]
      \path let \p0 = (begin highlight), \p1 = (0,0) in \pgfextra
        \global\highlight@previous=\y0
        \global\highlight@current =\y1
      \endpgfextra (0,0) ;
      \ifdim\highlight@current < \highlight@previous
        \highlight@DoHighlight
        \highlight@BeginHighlight
      \fi
    \end{tikzpicture}%
    \the\SOUL@syllable
    \tikz[overlay, remember picture] \highlight@EndHighlight ;%
  }%
  \SOUL@
}

\makeatother

\newcommand{\ie}{\emph{i.e.}\@\xspace}
\newcommand{\aka}{a.k.a.\@\xspace}
\newcommand{\Aka}{A.k.a.\@\xspace}
\newcommand{\Ie}{I.e.\@\xspace}
\newcommand{\cf}{cf.\@\xspace}
\newcommand{\Cf}{Cf.\@\xspace}
\newcommand{\eg}{\emph{e.g.}\@\xspace}
\newcommand{\Eg}{E.g.\@\xspace}
\newcommand{\etal}{\textit{et al.}\@\xspace}
\newcommand{\etc}{etc.\@\xspace}
\newcommand{\wrt}{\emph{w.r.t.}\@\xspace}
\newcommand{\Wrt}{W.r.t.\@\xspace}
\newcommand{\pom}{\textit{pom.xml}\@\xspace}
\newcommand{\tool}{\textsc{ToolName}\@\xspace}
\newcommand\duets{{\textsc{Duets}}\xspace}
\newcommand\proguard{{\sc Proguard}\xspace}
\newcommand\mv{{Maven}\xspace}
\newcommand\jar{\texttt{JAR}\xspace}
\newcommand\json{\texttt{json}\xspace}
\newcommand{\deptrim}{\textsc{DepTrim}\xspace}
\newcommand{\depclean}{\textsc{DepClean}\xspace}
\newcommand{\jshrink}{\textsc{JShrink}\xspace}
\newcommand{\nibbler}{\textsc{Nibbler}\xspace}
\newcommand{\molly}{\textsc{Molly}\xspace}
\newcommand{\shredder}{\textsc{Shredder}\xspace}
\newcommand{\buildmedic}{\textsc{BuildMedic}\xspace}
\newcommand{\stubbifier}{\textsc{Stubbifier}\xspace}
\newcommand{\libcapsule}{\textsc{LibCapsule}\xspace}
\newcommand{\trimmer}{\textsc{TRIMMER}\xspace}
\newcommand{\occam}{\textsc{OCCAM}\xspace}
\newcommand{\saffire}{\textsc{Saffire}\xspace}
\newtheorem{metric}{Metric}
\newcommand{\metricautorefname}{Metric}
\newtheorem{defn}{Definition}
\newcommand{\defnautorefname}{Definition}
\newcommand{\jacop}{\texttt{jacop}\@\xspace}
\newcommand{\maven}{\textsc{Maven}\@\xspace}
\newcommand{\tst}{\texttt{TST}\@\xspace}
\newcommand{\pst}{\texttt{PST}\@\xspace}
\newcommand{\cd}{\textsc{CD}\xspace}
\newcommand{\nbcd}{\textsc{NBCD}\xspace}
\newcommand{\compile}{\texttt{compile}\@\xspace}
\newcommand{\class}{\texttt{class}\@\xspace}
\newcommand{\tud}{\textsc{TUD}\xspace}
% ratio original
\newcommand{\ratioo}{\textsc{Ratio}$_\mathcal{O}$\@\xspace}
% ratio debloated
\newcommand{\ratiod}{\textsc{Ratio}$_\mathcal{D}$\@\xspace}
% ratio specialized
\newcommand{\ratios}{\textsc{Ratio}$_\mathcal{S}$\@\xspace}


==> utils/er.tex <==
% code for "one to omany", etc. is taken from https://tex.stackexchange.com/q/141797/101651
\makeatletter
\pgfarrowsdeclare{crow's foot}{crow's foot}
{
    \pgfarrowsleftextend{+-.5\pgflinewidth}%
    \pgfarrowsrightextend{+.5\pgflinewidth}%
}
{
    \pgfutil@tempdima=0.6pt%
    \pgfsetdash{}{+0pt}%
    \pgfsetmiterjoin%
    \pgfpathmoveto{\pgfqpoint{0pt}{-9\pgfutil@tempdima}}%
    \pgfpathlineto{\pgfqpoint{-13\pgfutil@tempdima}{0pt}}%
    \pgfpathlineto{\pgfqpoint{0pt}{9\pgfutil@tempdima}}%
    \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%
    \pgfpathmoveto{\pgfqpoint{-8pt}{-6pt}}% 
    \pgfpathlineto{\pgfqpoint{-8pt}{-6pt}}%  
    \pgfpathlineto{\pgfqpoint{-8pt}{6pt}}% 
    \pgfusepathqstroke%
}

\pgfarrowsdeclare{omany}{omany}
{
    \pgfarrowsleftextend{+-.5\pgflinewidth}%
    \pgfarrowsrightextend{+.5\pgflinewidth}%
}
{
    \pgfutil@tempdima=0.6pt%
    \pgfsetdash{}{+0pt}%
    \pgfsetmiterjoin%
    \pgfpathmoveto{\pgfqpoint{0pt}{-9\pgfutil@tempdima}}%
    \pgfpathlineto{\pgfqpoint{-13\pgfutil@tempdima}{0pt}}%
    \pgfpathlineto{\pgfqpoint{0pt}{9\pgfutil@tempdima}}%
    \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%  
    \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%
    \pgfpathmoveto{\pgfqpoint{-6pt}{-6pt}}% 
    \pgfusepathqstroke%
    \pgfsetfillcolor{white}
    \pgfpathcircle{\pgfpoint{-11.5pt}{0}} {3.5pt}
    \pgfusepathqfillstroke%
}

\pgfarrowsdeclare{one}{one}
{
    \pgfarrowsleftextend{+-.5\pgflinewidth}%
    \pgfarrowsrightextend{+.5\pgflinewidth}%
}
{
    \pgfutil@tempdima=0.6pt%
    \pgfsetdash{}{+0pt}%
    \pgfsetmiterjoin%
    \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%
    \pgfpathmoveto{\pgfqpoint{-6pt}{-6pt}}% 
    \pgfpathlineto{\pgfqpoint{-6pt}{-6pt}}%  
    \pgfpathlineto{\pgfqpoint{-6pt}{6pt}}% 
    \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%
    \pgfpathmoveto{\pgfqpoint{-8pt}{-6pt}}% 
    \pgfpathlineto{\pgfqpoint{-8pt}{-6pt}}%  
    \pgfpathlineto{\pgfqpoint{-8pt}{6pt}}%    
    \pgfusepathqstroke%
}

\pgfarrowsdeclare{oone}{oone}
{
    \pgfarrowsleftextend{+-.5\pgflinewidth}%
    \pgfarrowsrightextend{+.5\pgflinewidth}%
}
{
    \pgfutil@tempdima=0.6pt%
    %\advance\pgfutil@tempdima by.25\pgflinewidth%
    \pgfsetdash{}{+0pt}%
    \pgfsetmiterjoin%
     \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}%
    \
    pgfpathmoveto{\pgfqpoint{-4pt}{-6pt}}% 
    \pgfpathlineto{\pgfqpoint{-4pt}{-6pt}}%  
    \pgfpathlineto{\pgfqpoint{-4pt}{6pt}}% 
    \pgfsetfillcolor{white}
    \pgfpathcircle{\pgfpoint{-11.5pt}{0}} {3.5pt}
    \pgfusepathqfillstroke%
}
\makeatother

\tikzset{%
    mylabel/.style={font=\footnotesize},
    pics/entity/.style n args={3}{code={%
        \node[draw,
        rectangle split,
        rectangle split parts=2,
        text height=1.5ex,
        text width=7em,
        text centered
        ] (#1)
        {#2 \nodepart[font=\small, text centered]{second}
            \begin{tabular}{>{\raggedright\arraybackslash}p{9em}}
                #3
            \end{tabular}
        };%
    }},
    zig zag to/.style={
        to path={(\tikztostart) -| ($(\tikztostart)!#1!(\tikztotarget)$) |- (\tikztotarget)}
    },
    zig zag to/.default=0.5,   
    one to one/.style={
        one-one, zig zag to
    },
    one to oone/.style={% One to Optional-one
        one-oone, zig zag to
    },
    oone to none/.style={% Optional-one to none
        oone-, zig zag to
    },
    oone to oone/.style={% Optional one to Optional-one
        oone-oone, zig zag to
    },
    one to many/.style={
        one-crow's foot, zig zag to,
    },
    one to omany/.style={
        one-omany, zig zag to
    },
    one to none/.style={
        one-, zig zag to
    },   
    many to many/.style={
        crow's foot-crow's foot, zig zag to
    }
}

==> utils/macro.tex <==
\def\nbLib{94}
\def\nbLibStr{\np{\nbLib}}
\def\nbLibVersion{395}
\def\nbLibVersionStr{\np{\nbLibVersion}}
\def\nbLibCompiling{354}
\def\nbLibCompilingStr{\np{\nbLibCompiling}}
\def\nbTest{713932}
\def\nbTestStr{\np{\nbTest}}
\def\nbTestClient{211116}
\def\nbTestClientStr{\np{\nbTestClient}}
\def\nbClientAll{2874}
\def\nbClientAllStr{\np{\nbClientAll}}
\def\meanCoverageLib{73.73}
\def\meanCoverageLibStr{\np[\%]{\meanCoverageLib}}
\def\medianCoverageLib{80.83}
\def\medianCoverageLibStr{\np[\%]{\medianCoverageLib}}
\def\meanCoverageClient{31.17}
\def\meanCoverageClientStr{\np[\%]{\meanCoverageClient}}
\def\medianCoverageClient{20.24}
\def\medianCoverageClientStr{\np[\%]{\medianCoverageClient}}
\def\nbLineLib{10831394}
\def\nbLineLibStr{\np{\nbLineLib}}
\def\nbLineClient{140910102}
\def\nbLineClientStr{\np{\nbLineClient}}
\def\executionTime{4 days, 8:39:09\xspace}
\def\debloatTime{1 day, 10:55:04\xspace}

% RQ1
\def\nbLibDebSuccessNum{311}
\def\nbLibNotCompile{41}
\def\nbLibCrash{28}
\def\nbLibTimeout{13}
\def\nbLibValidation{2}

\def\debSuccessRate{\ShowPercentage{\nbLibDebSuccessNum}{\nbLibCompiling}}
\FPeval{nbDebloatError}{round(\nbLibVersion - \nbLibDebSuccessNum, 0)}


% RQ2
\def\nbLibDebSuccessNum{311}
\def\nbLibPassTestNum{220}
\def\nbLibExcludedForTest{61}
\def\nbLibTestFailing{30}
\def\nbUniqueTestNum{344596}
\def\nbTestForPassingNum{335222}
\def\nbFailingTest{1405}
\def\nbErrorTest{432}


\FPeval{nbLibExecTestNum}{round(\nbLibPassTestNum + \nbLibTestFailing, 0)}
\FPeval{nbPassingTestNum}{round(\nbUniqueTestNum - \nbFailingTest, 0)}
\FPeval{nbFailureTest}{round(\nbFailingTest - \nbErrorTest, 0)}

% RQ3

\def\nbLibWithDependencies{77}
\def\nbDependencies{254}
\def\nbClasses{121055}
\def\nbMethods{829015}
\def\nbBloatedDependencies{52}
\def\nbBloatedClasses{75273}
\def\nbBloatedMethods{505268}
\def\nbDepClasses{47765}
\def\nbDepMethods{367993}
\def\nbBloatedDepClasses{33391}
\def\nbPreservedDepClasses{0}
\def\nbBloatedDepMethods{254731}

\FPeval{nbLibWithoutDependencies}{round(\nbLibPassTestNum - \nbLibWithDependencies, 0)}
\FPeval{nbNonBloatedDependencies}{round(\nbDependencies - \nbBloatedDependencies, 0)}

% RQ4 
\def\totalSize{1151732283}
\def\resourceSize{257999869}
\def\bytecodeSize{893732414}
\def\debloatedSize{596538866}
\def\debloatedMethodSize{13768627}
\def\preservedSize{0}
\def\internalTotal{257772540}

\FPeval{bloatedSize}{round(\debloatedSize + \debloatedMethodSize, 0)}
\FPeval{nonBloatedSize}{round(\bytecodeSize - \debloatedSize - \debloatedMethodSize, 0)}

% RQ5 & RQ6
\def\nbClient{1370}
\def\nbCoveringClient{1066}
\def\nbDynCoveringClient{283}
\def\nbStatCoveringClient{1001}
\def\nbDifferentNbtest{3}
\def\nbFailingTestClient{54}
\def\nbFailingTestProject{39}
\def\nbClientTest{44428}
\def\nbClientFailure{744}
\def\nbClientDebloatError{44}
\def\nbClientDebloatCompilationError{43}
\def\nbClientDebloatPluginError{1}
\def\nbClientDebloatOtherError{0}
\def\nbClientConsideredPreserved{981}
\def\nbClientWithPreserved{0}

\def\nbTotalProject{147991}
\def\nbTotalProjectStr{\np{\nbTotalProject}}

\FPeval{nbCientDebloatNoCompError}{round(\nbStatCoveringClient - \nbClientDebloatError, 0)}
\FPeval{nbClientDebloatNoTestFail}{round(\nbDynCoveringClient - \nbFailingTestClient, 0)}


\FPeval{nbFailingTestNum}{round(\nbUniqueTestNum - \nbPassingTestNum, 0)}
\FPeval{nbSuccessTestNum}{round(\nbPassingTestNum*100/\nbUniqueTestNum, 2)}
\def\nbLibPassTest{\np{\nbLibPassTestNum}}
\FPeval{nbLibFailTestNum}{round(\nbLibDebSuccessNum - \nbLibPassTestNum, 0)}
\def\nbLibPassTestProportionNum{\ShowPercentage{\nbLibPassTestNum}{\nbLibDebSuccessNum}}


% --------------------------
% Custom commands
% --------------------------

% Percentage number
\newcommand{\percSizeReduction}{$XXX\%$\@\xspace}
\newcommand{\percClassesReduction}{$XXX\%$\@\xspace}






==> utils/percentage.tex <==
% This command is to right align an integer number so that the numbers in the column of the table are all right-aligned
\newcommand{\ShowAbsoluteNumber}[1]{%
\ifnum #1<10%
{\hspace*{0pt}#1}%
\else%
\ifnum #1<100%
{\hspace*{0pt}#1}%
\else%
\ifnum #1<1000%
{\hspace*{0pt}#1}%
\else%
{\numprint{#1}}%
\fi%
\fi%
\fi%
}

% This command is to calculate a percentage given a number and the total number, and to present it between parentheses where the percentage number itself is right-aligned so that the left parentheses in the column of the table are all left-aligned. Note that a percentage rounded to 0 will be presented as <1%
\newcommand{\ShowPercentage}[2]{%
\FPeval\percentage{round(#1/#2*10000,0)}%
%\FPeval\percentage{#1/#2*100}%
\FPeval\percentageOneDecimal{round(#1/#2*100,1)}%
\ifnum \percentage=0%
    {\np[\%]{0}}%
\else%
    \ifnum \percentage<10%
        {$<$\np[\%]{0.1}}%
    \else%
        {\np[\%]{\FPprint{percentageOneDecimal}}}%
    \fi%
\fi%
\xspace
}
\newlength\BARSIZE  \setlength\BARSIZE{0.5cm}
\newcommand{\inlinechart}[2]{%
\FPeval{\BLACKBARSIZE}{#1/#2}\textcolor{black!80}{\rule{\BLACKBARSIZE\BARSIZE}{1.6ex}}%
\FPeval{\BLACKBARSIZE}{1 - (#1/#2)}\textcolor{black!10}{\rule{\BLACKBARSIZE\BARSIZE}{1.6ex}}%
}

\newcommand*\ChartSmall[3][v]{%
\ifx q#1%
    \np{#2}/\np{#3}(\ShowPercentage{#2}{#3})\else%
\ifx p#1%
    \np{#2}(\ShowPercentage{#2}{#3})
\ifx c#1%
    \np{#2}/\np{#3}
\else%
    \np{#2}%
    \ifx r#1%
        /\np{#3}%
    \fi%
    \hspace*{0.5ex}(\ShowPercentage{#2}{#3}) %
    \inlinechart{#2}{#3}%
    \xspace
\fi\fi\fi%
}




==> zero-class-dependencies.tex <==
1
checkstyle
com.google.guava:listenablefuture:9999.0-empty-to-avoid-conflict-with-guava
listenablefuture-9999.0-empty-to-avoid-conflict-with-guava
0
2
jooby_jooby
org.jetbrains.kotlinx:kotlinx-coroutines-core:1.6.2
kotlinx-coroutines-core-1.6.2
0
3
jooby_jooby
org.jetbrains.kotlin:kotlin-stdlib-common:1.6.21
kotlin-stdlib-common-1.6.21
0
4
flink
org.apache.flink:flink-shaded-force-shading:15.0
flink-shaded-force-shading-15.0
0
5
lettuce-core
io.netty:netty-transport-native-epoll:4.1.85.Final
netty-transport-native-epoll-4.1.85.Final-linux-x86_64
0
6
lettuce-core
io.netty:netty-tcnative:2.0.54.Final
netty-tcnative-2.0.54.Final-linux-x86_64
0
7
lettuce-core
org.jetbrains.kotlin:kotlin-stdlib-common:1.5.30
kotlin-stdlib-common-1.5.30
0
8
lettuce-core
io.netty:netty-transport-native-kqueue:4.1.85.Final
netty-transport-native-kqueue-4.1.85.Final-osx-x86_64
0
9
lettuce-core
io.netty.incubator:netty-incubator-transport-native-io_uring:0.0.16.Final
netty-incubator-transport-native-io_uring-0.0.16.Final-linux-x86_64
0
10
guice
com.google.guava:listenablefuture:9999.0-empty-to-avoid-conflict-with-guava
listenablefuture-9999.0-empty-to-avoid-conflict-with-guava
0
11
Recaf
com.google.guava:listenablefuture:9999.0-empty-to-avoid-conflict-with-guava
listenablefuture-9999.0-empty-to-avoid-conflict-with-guava
0
12
jimfs
com.google.guava:listenablefuture:9999.0-empty-to-avoid-conflict-with-guava
listenablefuture-9999.0-empty-to-avoid-conflict-with-guava
0
13
OpenPDF
org.apache.xmlgraphics:batik-shared-resources:1.14
batik-shared-resources-1.14
0
14
jcabi-github
com.google.guava:listenablefuture:9999.0-empty-to-avoid-conflict-with-guava
listenablefuture-9999.0-empty-to-avoid-conflict-with-guava
0
15
poi-tl
org.apache.xmlgraphics:batik-shared-resources:1.14
batik-shared-resources-1.14
0
